Mapping Active Star-Formation in Serpens and the Aquila Rift

We report the results of a high-sensitivity survey for Herbig-Haro (HH) outflows in the Serpens-Aquila Rift using the DECam instrument on the 4-meter telescope. We have detected 88 new HH objects, more than tripling the total known in this region. We have also identified likely progenitors for most of these outflows. By combining HH object and progenitor locations with literature dust maps and Gaia astrometry, we find that HH objects mark five spatially distinct clouds hosting active star formation: the Serpens Molecular Cloud and LDN 673 at 400-500 pc, the more distant West and East components of the Aquila Rift at ~600 and 700 pc, respectively, and a near cloud in Serpens at ~250 pc. In both the Serpens Molecular Cloud and the Western Aquila Rift, HH objects broadly trace gas structures on the edges of low-density cavities surrounding known stellar populations, consistent with active star formation in feedback-driven shells. The near cloud in Serpens is not associated with any established stellar population, but its position and velocity suggest that it is part of the Local Bubble. And the HH objects there may mark the start of a new stellar generation connected to the Scutum North Association. Our Herbig-Haro objects therefore serve as a powerful indicator of star formation sites even in the absence of astrometrically characterized young stars, making them a useful tool for guiding future YSO surveys.

==> allwise_matches.tex <==
\startlongtable
\begin{deluxetable*}{llccccc}
\tablecaption{Matching AllWISE Sources \label{tbl:allwise_matches}}
\tablewidth{0pt}
\tablehead{
\colhead{Input Source} &
\colhead{AllWISE Designation} &
\colhead{$W1-W2$} &
\colhead{$\sigma$} &
\colhead{$W2-W3$} &
\colhead{$\sigma$} &
\colhead{Sp. Class}
}
\startdata
DAB2006 MMS1 & J182854.05+002929.4 & 3.167 & 0.018 & 2.756 & 0.023 & I \\
GE91 GGD 30 I1 & J185140.46+002858.1 & 2.395 & 0.057 & 1.736 & 0.059 & Im \\
2MASS J18251133-0258532 & J182511.34-025853.4 & 2.839 & 0.028 & 4.377 & 0.033 & I \\
2MASS J18251332-0259549 & J182513.32-025954.9 & 1.644 & 0.020 & 2.222 & 0.026 & I \\
2MASS J18300341+0116191 & J183003.42+011618.7 & 0.522 & 0.019 & 2.628 & 0.023 & II \\
2MASS J18391236-0720158 & J183912.30-072014.2 & 0.547 & 0.025 & 1.535 & 0.184 & II \\
2MASS J18494869+0006072 & J184949.20+000605.5 & 0.314 & 0.033 & \nodata & \nodata & N/A \\
AGAL G034.196-00.592 & J185551.22+005120.3 & 1.463 & 0.019 & 4.318 & 0.021 & I \\
EM* AS  353 & J192030.99+110153.5 & 0.924 & 0.077 & 1.689 & 0.078 & II \\
SSTc2d J192031.0+110149 & J192030.99+110153.5 & 0.924 & 0.077 & 1.689 & 0.078 & II \\
SSTc2d J192031.9+110151 & J192031.87+110150.7 & 1.062 & 0.026 & 3.004 & 0.033 & I \\
CORNISH G039.1956+00.2255 & J190205.63+054031.5 & 1.726 & 0.022 & 5.166 & 0.027 & other \\
DLW84 G35.2N & J185813.06+014038.8 & 3.479 & 0.026 & 3.436 & 0.032 & I \\
2MASS J19070986+0513107 & J190709.86+051310.7 & 1.369 & 0.055 & 2.502 & 0.057 & I \\
HGBS J183629.6-022159 & J183629.54-022158.4 & 2.555 & 0.020 & 3.371 & 0.025 & I \\
HIGALBM G034.3395-00.6940 & J185628.74+005608.5 & 1.507 & 0.020 & 2.348 & 0.028 & I \\
HIGALBM G034.3721-00.5424 & J185559.90+010203.7 & 1.902 & 0.021 & 2.973 & 0.030 & I \\
HIGALBM G038.6940+00.4527 & J190021.57+052001.2 & 1.921 & 0.022 & 2.416 & 0.027 & I \\
IRAS 18148-0440 & J181730.02-043939.7 & 3.184 & 0.021 & 1.105 & 0.028 & other \\
IRAS 18197-0158 & J182222.28-015659.5 & 1.702 & 0.069 & 2.642 & 0.070 & I \\
IRAS 18264-0143 & J182905.32-014156.5 & 2.403 & 0.019 & 1.778 & 0.025 & Im \\
IRAS 18268-0140 & J182923.39-013855.4 & 2.516 & 0.019 & 3.313 & 0.024 & I \\
IRAS 18269+0116 & J182931.98+011842.5 & 1.520 & 0.073 & 2.408 & 0.074 & I \\
GCNM  23 & J182949.65+011521.6 & 4.527 & 0.021 & 1.054 & 0.051 & other \\
IRAS 18301+0035 & J183239.15+003753.2 & 0.892 & 0.023 & 1.774 & 0.045 & II \\
IRAS 18327-0645 & J183524.35-064259.2 & 3.456 & 0.061 & 4.488 & 0.079 & I \\
IRAS 18331-0035 & J183542.08-003320.3 & 2.193 & 0.020 & \nodata & \nodata & N/A \\
IRAS 18358-0112 & J183826.27-010950.9 & 4.024 & 0.019 & 2.409 & 0.028 & I \\
IRAS 18383+0059 & J184051.78+010212.9 & 1.763 & 0.028 & 2.421 & 0.031 & I \\
IRAS 18440+0023 & J184632.22+002708.5 & 1.961 & 0.020 & 2.698 & 0.025 & I \\
IRAS 18454+0250 & J184800.65+025417.2 & 0.975 & 0.055 & 2.860 & 0.056 & II \\
IRAS 18484+0237 & J185057.46+024051.8 & 1.611 & 0.020 & 2.777 & 0.027 & I \\
IRAS 18528+0400 & J185522.97+040435.1 & 1.263 & 0.039 & 2.517 & 0.042 & I \\
IRAS 18542+0114 & J185648.26+011846.9 & 2.807 & 0.217 & 2.170 & 0.219 & I \\
IRAS 18550+0104 & J185736.93+010807.9 & 1.650 & 0.225 & 2.003 & 0.228 & I \\
IRAS 18555+0056 & J185808.47+010041.3 & 2.952 & 0.091 & 3.210 & 0.112 & I \\
IRAS 18558+0047 & J185823.96+005153.5 & 1.139 & 0.019 & 2.500 & 0.024 & II \\
IRAS 18566+0048 & J185913.05+005239.1 & 2.873 & 0.020 & 3.324 & 0.026 & I \\
IRAS 18589+0511 & J190126.55+051526.3 & 1.879 & 0.024 & 3.096 & 0.028 & I \\
IRAS 18591+0503 & J190135.25+050746.7 & \nodata & \nodata & 5.156 & 0.064 & N/A \\
IRAS 19045+0518 & J190659.73+052255.1 & 2.135 & 0.075 & 2.807 & 0.077 & I \\
IRAS 19158+1136 & J191812.33+114153.0 & 2.372 & 0.021 & 4.437 & 0.025 & I \\
IRAS 19160+1139 & J191825.87+114451.0 & 2.368 & 0.046 & 1.860 & 0.048 & Im \\
NAME HH 250-IRS & J192122.62+105357.0 & 1.694 & 0.024 & 2.825 & 0.028 & I \\
MSX6C G034.0126-00.2832 & J185425.06+004956.4 & 2.030 & 0.145 & 2.243 & 0.150 & I \\
MSX6C G034.0500-00.2977 & J185432.27+005132.3 & 0.853 & 0.024 & 4.086 & 0.039 & other \\
SPICY 87918 & J183638.78-011330.1 & 2.539 & 0.049 & 2.623 & 0.081 & I \\
2MASS J18364058-0112053 & J183640.58-011204.2 & 1.725 & 0.024 & 2.913 & 0.070 & I \\
SPICY 92856 & J184948.94+000627.9 & 1.467 & 0.056 & \nodata & \nodata & N/A \\
SPICY 92890 & J184952.82+001253.5 & 0.118 & 0.069 & \nodata & \nodata & N/A \\
SPICY 92905 & J184956.28+001121.2 & 3.629 & 0.030 & 2.462 & 0.055 & I \\
SSTc2d J192025.8+111959 & J192026.00+111952.4 & 1.870 & 0.019 & 2.130 & 0.028 & I \\
TBP2010 L673 10 & J192026.00+111952.4 & 1.870 & 0.019 & 2.130 & 0.028 & I \\
2MASS J19202603+1119525 & J192026.00+111952.4 & 1.870 & 0.019 & 2.130 & 0.028 & I \\
2MASS J19202598+1120084 & J192025.97+112007.5 & 2.242 & 0.021 & 0.602 & 0.253 & other \\
2MASS J19202616+1119491 & J192026.00+111952.4 & 1.870 & 0.019 & 2.130 & 0.028 & I \\
2MASS J19202706+1120109 & J192027.06+112011.0 & 2.412 & 0.019 & 2.274 & 0.029 & I \\
SSTGLMC G025.2255+00.2884 & J183616.87-064318.2 & 1.030 & 0.022 & 1.861 & 0.039 & II \\
\enddata
\tablecomments{Spectral Class derived from color-color classification scheme in \citet{Fischer+2016}. ``N/A'' indicates sources lacking reliable photometry in one or more bands.}
\end{deluxetable*}

==> appfigs.tex <==
\begin{figure}
\gridline{\fig{aql_f01_A_giha.pdf}{0.33\textwidth}{HH1358}
          \fig{aql_f01_A_s2.pdf}{0.33\textwidth}{HH1358}
          }
\gridline{\fig{aql_f01_B_giha.pdf}{0.33\textwidth}{HH1361}
          \fig{aql_f01_B_s2.pdf}{0.33\textwidth}{HH1361}
          }
\gridline{\fig{aql_f01_C_giha.pdf}{0.33\textwidth}{HH1360}
          \fig{aql_f01_C_s2.pdf}{0.33\textwidth}{HH1360}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f01_F_giha.pdf}{0.33\textwidth}{Aql\_f01\_F}
          \fig{aql_f01_F_s2.pdf}{0.33\textwidth}{Aql\_f01\_F}
          }
\gridline{\fig{aql_f02pt5_A_giha.pdf}{0.33\textwidth}{Aql\_f02.5\_A}
          }
\gridline{\fig{aql_f03pt5_A_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_A}
          \fig{aql_f03pt5_A_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_B_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_B}
          \fig{aql_f03pt5_B_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_B}
          }
\gridline{\fig{aql_f03pt5_C_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_C}
          \fig{aql_f03pt5_C_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_C}
          }
\gridline{\fig{aql_f03pt5_D_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_D}
          \fig{aql_f03pt5_D_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_EF_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_E \& F}
          \fig{aql_f03pt5_EF_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_E \& F}
          }
\gridline{\fig{aql_f03pt5_G_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_G}
          \fig{aql_f03pt5_G_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_G}
          }
\gridline{\fig{aql_f03pt5_H_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_H}
          \fig{aql_f03pt5_H_s2.pdf}{0.33\textwidth}{Aql\_f\_f03.5\_H}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_I_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_I}
          \fig{aql_f03pt5_I_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_I}
          }
\gridline{\fig{aql_f03pt5_L_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_L}
          \fig{aql_f03pt5_L_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_L}
          }
\gridline{\fig{aql_f03pt5_M_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_M}
          \fig{aql_f03pt5_M_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_M}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_N_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_N}
          \fig{aql_f03pt5_N_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_N}
          }
\gridline{\fig{aql_f03pt5_O_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_O}
          \fig{aql_f03pt5_O_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_O}
          }
\gridline{\fig{aql_f03pt5_P_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_P}
          \fig{aql_f03pt5_P_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_P}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_Q_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_Q}
          \fig{aql_f03pt5_Q_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_Q}
          }
\gridline{\fig{aql_f03pt5_R_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_R}
          \fig{aql_f03pt5_R_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_R}
          }
\gridline{\fig{aql_f03pt5_S_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_S}
          \fig{aql_f03pt5_S_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_S}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_f03pt5_T_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_T}
          \fig{aql_f03pt5_T_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_T}
          }
\gridline{\fig{aql_f03pt5_U_giha.pdf}{0.33\textwidth}{Aql\_f03.5\_U}
          \fig{aql_f03pt5_U_s2.pdf}{0.33\textwidth}{Aql\_f03.5\_U}
          }
\gridline{\fig{aql_nf01_A_giha.pdf}{0.33\textwidth}{Aql\_nf01\_A}
          \fig{aql_nf01_A_s2.pdf}{0.33\textwidth}{Aql\_nf01\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf01_B_giha.pdf}{0.33\textwidth}{Aql\_nf01\_B}
          \fig{aql_nf01_B_s2.pdf}{0.33\textwidth}{Aql\_nf01\_B}
          }
\gridline{\fig{aql_nf01_C_giha.pdf}{0.33\textwidth}{Aql\_nf01\_C}
          \fig{aql_nf01_C_s2.pdf}{0.33\textwidth}{Aql\_nf01\_C}
          }
\gridline{\fig{aql_nf01_D_giha.pdf}{0.33\textwidth}{Aql\_nf01\_D}
          \fig{aql_nf01_D_s2.pdf}{0.33\textwidth}{Aql\_nf01\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf01_E_giha.pdf}{0.33\textwidth}{Aql\_nf01\_E}
          \fig{aql_nf01_E_s2.pdf}{0.33\textwidth}{Aql\_nf01\_E}
          }
\gridline{\fig{aql_nf01_F_giha.pdf}{0.33\textwidth}{Aql\_nf01\_F}
          \fig{aql_nf01_F_s2.pdf}{0.33\textwidth}{Aql\_nf01\_F}
          }
\gridline{\fig{aql_nf01_G_giha.pdf}{0.33\textwidth}{Aql\_nf01\_G}
          \fig{aql_nf01_G_s2.pdf}{0.33\textwidth}{Aql\_nf01\_G}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf03_B_giha.pdf}{0.33\textwidth}{Aql\_nf03\_B}
          \fig{aql_nf03_B_s2.pdf}{0.33\textwidth}{Aql\_nf03\_B}
          }
\gridline{\fig{aql_nf03_C_giha.pdf}{0.33\textwidth}{Aql\_nf03\_C}
          \fig{aql_nf03_C_s2.pdf}{0.33\textwidth}{Aql\_nf03\_C}
          }
\gridline{\fig{aql_nf03_D_giha.pdf}{0.33\textwidth}{Aql\_nf03\_D}
          \fig{aql_nf03_D_s2.pdf}{0.33\textwidth}{Aql\_nf03\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf03_E_giha.pdf}{0.33\textwidth}{Aql\_nf03\_E}
          \fig{aql_nf03_E_s2.pdf}{0.33\textwidth}{Aql\_nf03\_E}
          }
\gridline{\fig{aql_nf03_F_giha.pdf}{0.33\textwidth}{Aql\_nf03\_F}
          \fig{aql_nf03_F_s2.pdf}{0.33\textwidth}{Aql\_nf03\_F}
          }
\gridline{\fig{aql_nf03_G_giha.pdf}{0.33\textwidth}{Aql\_nf03\_G}
          \fig{aql_nf03_G_s2.pdf}{0.33\textwidth}{Aql\_nf03\_G}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf03_H_giha.pdf}{0.33\textwidth}{Aql\_nf03\_H}
          \fig{aql_nf03_H_s2.pdf}{0.33\textwidth}{Aql\_nf03\_H}
          }
\gridline{\fig{aql_nf03_I_giha.pdf}{0.33\textwidth}{Aql\_nf03\_I}
          \fig{aql_nf03_I_s2.pdf}{0.33\textwidth}{Aql\_nf03\_I}
          }
\gridline{\fig{aql_nf03_J_giha.pdf}{0.33\textwidth}{Aql\_nf03\_J}
          \fig{aql_nf03_J_s2.pdf}{0.33\textwidth}{Aql\_nf03\_J}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf03_K_giha.pdf}{0.33\textwidth}{Aql\_nf03\_K}
          \fig{aql_nf03_K_s2.pdf}{0.33\textwidth}{Aql\_nf03\_K}
          }
\gridline{\fig{aql_nf06_A_giha.pdf}{0.33\textwidth}{Aql\_nf06\_A}
          \fig{aql_nf06_A_s2.pdf}{0.33\textwidth}{Aql\_nf06\_A}
          }
\gridline{\fig{aql_nf06_CD_giha.pdf}{0.33\textwidth}{Aql\_nf06\_CD}
          \fig{aql_nf06_CD_s2.pdf}{0.33\textwidth}{Aql\_nf06\_CD}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf06_F_giha.pdf}{0.33\textwidth}{Aql\_nf06\_F}
          \fig{aql_nf06_F_s2.pdf}{0.33\textwidth}{Aql\_nf06\_F}
          }
\gridline{\fig{aql_nf06_G_giha.pdf}{0.33\textwidth}{Aql\_nf06\_G}
          \fig{aql_nf06_G_s2.pdf}{0.33\textwidth}{Aql\_nf06\_G}
          }
\gridline{\fig{aql_nf06_H_giha.pdf}{0.33\textwidth}{Aql\_nf06\_H}
          \fig{aql_nf06_H_s2.pdf}{0.33\textwidth}{Aql\_nf06\_H}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf06_J_giha.pdf}{0.33\textwidth}{Aql\_nf06\_J}
          \fig{aql_nf06_J_s2.pdf}{0.33\textwidth}{Aql\_nf06\_J}
          }
\gridline{\fig{aql_nf06_N_giha.pdf}{0.33\textwidth}{Aql\_nf06\_N}
          \fig{aql_nf06_N_s2.pdf}{0.33\textwidth}{Aql\_nf06\_N}
          }
\gridline{\fig{aql_nf07_A_giha.pdf}{0.33\textwidth}{Aql\_nf07\_A}
          \fig{aql_nf07_A_s2.pdf}{0.33\textwidth}{Aql\_nf07\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf07_B_giha.pdf}{0.33\textwidth}{Aql\_nf07\_B}
          \fig{aql_nf07_B_s2.pdf}{0.33\textwidth}{Aql\_nf07\_B}
          }
\gridline{\fig{aql_nf07_C_giha.pdf}{0.33\textwidth}{Aql\_nf07\_C}
          \fig{aql_nf07_C_s2.pdf}{0.33\textwidth}{Aql\_nf07\_C}
          }
\gridline{\fig{aql_nf07_D_giha.pdf}{0.33\textwidth}{Aql\_nf07\_D}
          \fig{aql_nf07_D_s2.pdf}{0.33\textwidth}{Aql\_nf07\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf07_G_giha.pdf}{0.33\textwidth}{Aql\_nf07\_G}
          \fig{aql_nf07_G_s2.pdf}{0.33\textwidth}{Aql\_nf07\_G}
          }
\gridline{\fig{aql_nf08_A_giha.pdf}{0.33\textwidth}{Aql\_nf08\_A}
          \fig{aql_nf08_A_s2.pdf}{0.33\textwidth}{Aql\_nf08\_A}
          }
\gridline{\fig{aql_nf08_BC_giha.pdf}{0.33\textwidth}{Aql\_nf08\_B \& C}
          \fig{aql_nf08_BC_s2.pdf}{0.33\textwidth}{Aql\_nf08\_B \& C}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf08_D_giha.pdf}{0.33\textwidth}{Aql\_nf08\_D}
          \fig{aql_nf08_D_s2.pdf}{0.33\textwidth}{Aql\_nf08\_D}
          }
\gridline{\fig{aql_nf10_A_giha.pdf}{0.33\textwidth}{Aql\_nf10\_A}
          \fig{aql_nf10_A_s2.pdf}{0.33\textwidth}{Aql\_nf10\_A}
          }
\gridline{\fig{aql_nf10_B_giha.pdf}{0.33\textwidth}{Aql\_nf10\_B}
          \fig{aql_nf10_B_s2.pdf}{0.33\textwidth}{Aql\_nf10\_B}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf10_C_giha.pdf}{0.33\textwidth}{Aql\_nf10\_C}
          \fig{aql_nf10_C_s2.pdf}{0.33\textwidth}{Aql\_nf10\_C}
          }
\gridline{\fig{aql_nf10_D_giha.pdf}{0.33\textwidth}{Aql\_nf10\_D}
          \fig{aql_nf10_D_s2.pdf}{0.33\textwidth}{Aql\_nf10\_D}
          }
\gridline{\fig{aql_nf10_EF_giha.pdf}{0.33\textwidth}{Aql\_nf10\_E \& F}
          \fig{aql_nf10_EF_s2.pdf}{0.33\textwidth}{Aql\_nf10\_E \& F}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf10_G_giha.pdf}{0.33\textwidth}{Aql\_nf10\_G}
          \fig{aql_nf10_G_s2.pdf}{0.33\textwidth}{Aql\_nf10\_G}
          }
\gridline{\fig{aql_nf10_H_giha.pdf}{0.33\textwidth}{Aql\_nf10\_H}
          \fig{aql_nf10_H_s2.pdf}{0.33\textwidth}{Aql\_nf10\_H}
          }
\gridline{\fig{aql_nf11_A_giha.pdf}{0.33\textwidth}{Aql\_nf11\_A}
          \fig{aql_nf11_A_s2.pdf}{0.33\textwidth}{Aql\_nf11\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf11_B_giha.pdf}{0.33\textwidth}{Aql\_nf11\_B}
          \fig{aql_nf11_B_s2.pdf}{0.33\textwidth}{Aql\_nf11\_B}
          }
\gridline{\fig{aql_nf11_C_giha.pdf}{0.33\textwidth}{Aql\_nf11\_C}
          \fig{aql_nf11_C_s2.pdf}{0.33\textwidth}{Aql\_nf11\_C}
          }
\gridline{\fig{aql_nf12_A_giha.pdf}{0.33\textwidth}{Aql\_nf12\_A}
          \fig{aql_nf12_A_s2.pdf}{0.33\textwidth}{Aql\_nf12\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf12_B_giha.pdf}{0.33\textwidth}{Aql\_nf12\_B}
          \fig{aql_nf12_B_s2.pdf}{0.33\textwidth}{Aql\_nf12\_B}
          }
\gridline{\fig{aql_nf12_C_giha.pdf}{0.33\textwidth}{Aql\_nf12\_C}
          \fig{aql_nf12_C_s2.pdf}{0.33\textwidth}{Aql\_nf12\_C}
          }
\gridline{\fig{aql_nf12_D_giha.pdf}{0.33\textwidth}{Aql\_nf12\_D}
          \fig{aql_nf12_D_s2.pdf}{0.33\textwidth}{Aql\_nf12\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf12_E_giha.pdf}{0.33\textwidth}{Aql\_nf12\_E}
          \fig{aql_nf12_E_s2.pdf}{0.33\textwidth}{Aql\_nf12\_E}
          }
\gridline{\fig{aql_nf13_AB_giha.pdf}{0.33\textwidth}{Aql\_nf13\_A \& B}
          \fig{aql_nf13_AB_s2.pdf}{0.33\textwidth}{Aql\_nf13\_A \& B}
          }
\gridline{\fig{aql_nf13_C_giha.pdf}{0.33\textwidth}{Aql\_nf13\_C}
          \fig{aql_nf13_C_s2.pdf}{0.33\textwidth}{Aql\_nf13\_C}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf13_D_giha.pdf}{0.33\textwidth}{Aql\_nf13\_D}
          \fig{aql_nf13_D_s2.pdf}{0.33\textwidth}{Aql\_nf13\_D}
          }
\gridline{\fig{aql_nf13_E_giha.pdf}{0.33\textwidth}{Aql\_nf13\_E}
          \fig{aql_nf13_E_s2.pdf}{0.33\textwidth}{Aql\_nf13\_E}
          }
\gridline{\fig{aql_nf13_G_giha.pdf}{0.33\textwidth}{Aql\_nf13\_G}
          \fig{aql_nf13_G_s2.pdf}{0.33\textwidth}{Aql\_nf13\_G}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf13_HI_giha.pdf}{0.33\textwidth}{Aql\_nf13\_H \& I}
          \fig{aql_nf13_HI_s2.pdf}{0.33\textwidth}{Aql\_nf13\_H \& I}
          }
\gridline{\fig{aql_nf13_J_giha.pdf}{0.33\textwidth}{Aql\_nf13\_J}
          \fig{aql_nf13_J_s2.pdf}{0.33\textwidth}{Aql\_nf13\_J}
          }
\gridline{\fig{aql_nf23_F_giha.pdf}{0.33\textwidth}{Aql\_nf23\_F}
          \fig{aql_nf23_F_s2.pdf}{0.33\textwidth}{Aql\_nf23\_F}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf26_A_giha.pdf}{0.33\textwidth}{Aql\_nf26\_A}
          \fig{aql_nf26_A_s2.pdf}{0.33\textwidth}{Aql\_nf26\_A}
          }
\gridline{\fig{aql_nf26_B_giha.pdf}{0.33\textwidth}{Aql\_nf26\_B}
          \fig{aql_nf26_B_s2.pdf}{0.33\textwidth}{Aql\_nf26\_B}
          }
\gridline{\fig{aql_nf33_A_giha.pdf}{0.33\textwidth}{Aql\_nf33\_A}
          \fig{aql_nf33_A_s2.pdf}{0.33\textwidth}{Aql\_nf33\_A}
          }
\end{figure}

\begin{figure}
\gridline{\fig{aql_nf33_C_giha.pdf}{0.33\textwidth}{Aql\_nf33\_C}
          \fig{aql_nf33_C_s2.pdf}{0.33\textwidth}{Aql\_nf33\_C}
          }
\gridline{\fig{aql_nf33_D_giha.pdf}{0.33\textwidth}{Aql\_nf33\_D}
          \fig{aql_nf33_D_s2.pdf}{0.33\textwidth}{Aql\_nf33\_D}
          }
\end{figure}

\begin{figure}
\gridline{\fig{hh106_giha.pdf}{0.33\textwidth}{HH 106}
          \fig{hh106_s2.pdf}{0.33\textwidth}{HH 106}
          }
\gridline{\fig{hh107_giha.pdf}{0.33\textwidth}{HH 107}
          \fig{hh107_s2.pdf}{0.33\textwidth}{HH 107}
          }
\gridline{\fig{hh108y109_giha.pdf}{0.33\textwidth}{HH 108 \& 109}
          }
\end{figure}

\begin{figure}
\gridline{\fig{hh250_giha.pdf}{0.33\textwidth}{HH 250}
          \fig{hh250_s2.pdf}{0.33\textwidth}{HH 250}
          }
\gridline{\fig{hh455_giha.pdf}{0.33\textwidth}{HH 455}
          \fig{hh455_s2.pdf}{0.33\textwidth}{HH 455}
          }
\gridline{\fig{hh458-9_giha.pdf}{0.33\textwidth}{HH 458 \& 459}
          \fig{hh458-9_s2.pdf}{0.33\textwidth}{HH 458 \& 459}
          }
\end{figure}

\begin{figure}
\gridline{\fig{hh460_giha.pdf}{0.33\textwidth}{HH 460}
          \fig{hh460_s2.pdf}{0.33\textwidth}{HH 460}
          }
\gridline{\fig{hh476_giha.pdf}{0.33\textwidth}{HH 476}
          \fig{hh476_s2.pdf}{0.33\textwidth}{HH 476}
          }
\gridline{\fig{hh477_giha.pdf}{0.33\textwidth}{HH 477}
          \fig{hh477_s2.pdf}{0.33\textwidth}{HH 477}
          }
\end{figure}

\begin{figure}
\gridline{\fig{hh478_giha.pdf}{0.33\textwidth}{HH 478}
          \fig{hh478_s2.pdf}{0.33\textwidth}{HH 478}
          }
\gridline{\fig{hh721y724_giha.pdf}{0.33\textwidth}{HH 721 \& 724}
          \fig{hh721y724_s2.pdf}{0.33\textwidth}{HH 721 \& 724}
          }
\gridline{\fig{hh722_giha.pdf}{0.33\textwidth}{HH 722}
          \fig{hh722_s2.pdf}{0.33\textwidth}{HH 722}
          }
\end{figure}

\begin{figure}
\gridline{\fig{hh723_giha.pdf}{0.33\textwidth}{HH 723}
          \fig{hh723_s2.pdf}{0.33\textwidth}{HH 723}
          }
\end{figure}

==> figure_set_v2.tex <==
%% You can integrate this mark up directly into your ms.tex file
%% by placing the new commands below before your \begin{document}
%% command and everything that follows within the run of text 
%% where you want the figure set to appear.
%\documentclass[12pt,preprint]{aastex}
 
% FIGSET-MACROS-BEGIN
%\newcommand{\noprint}[1]{}
%\newcommand{\figsetstart}{{\bf Fig. Set} }
%\newcommand{\figsetend}{}
%\newcommand{\figsetgrpstart}{}
%\newcommand{\figsetgrpend}{}
%\newcommand{\figsetnum}[1]{{\bf #1.}}
%\newcommand{\figsettitle}[1]{ {\bf #1} }
%\newcommand{\figsetgrpnum}[1]{\noprint{#1}}
%\newcommand{\figsetgrptitle}[1]{\noprint{#1}}
%\newcommand{\figsetplot}[1]{\noprint{#1}}
%\newcommand{\figsetgrpnote}[1]{\noprint{#1}}
% FIGSET-MACROS-END
 
%\begin{document}

\figsetstart
\figsetnum{2}
\figsettitle{Cutouts for HH Objects}

\figsetgrpstart
\figsetgrpnum{2.1}
\figsetgrptitle{HH106 (g,i,H$\alpha$)
}
\figsetplot{hh106_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.2}
\figsetgrptitle{HH106 ([SII])
}
\figsetplot{hh106_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.3}
\figsetgrptitle{HH107 (g,i,H$\alpha$)
}
\figsetplot{hh107_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.4}
\figsetgrptitle{HH107 ([SII])
}
\figsetplot{hh107_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.5}
\figsetgrptitle{HH107B (g,i,H$\alpha$)
}
\figsetplot{hh107B_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.6}
\figsetgrptitle{HH107B ([SII])
}
\figsetplot{hh107B_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.7}
\figsetgrptitle{HH108 \& HH109 (g,i,H$\alpha$)
}
\figsetplot{hh108y109_giha.pdf}
\figsetgrpnote{HH108 is in the lower left; HH109 in the upper right. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.8}
\figsetgrptitle{HH172 (g,i,H$\alpha$)
}
\figsetplot{hh172_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.9}
\figsetgrptitle{HH172 ([SII])
}
\figsetplot{hh172_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.10}
\figsetgrptitle{HH250 (g,i,H$\alpha$)
}
\figsetplot{hh250_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.11}
\figsetgrptitle{HH250 ([SII])
}
\figsetplot{hh250_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.12}
\figsetgrptitle{HH455 (g,i,H$\alpha$)
}
\figsetplot{hh455_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.13}
\figsetgrptitle{HH455 ([SII])
}
\figsetplot{hh455_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.14}
\figsetgrptitle{HH456-7 (g,i,H$\alpha$)
}
\figsetplot{hh456-7_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.15}
\figsetgrptitle{HH456-7 ([SII])
}
\figsetplot{hh456-7_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.16}
\figsetgrptitle{HH458-9 (g,i,H$\alpha$)
}
\figsetplot{hh458-9_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.17}
\figsetgrptitle{HH458-9 ([SII])
}
\figsetplot{hh458-9_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.18}
\figsetgrptitle{HH460 (g,i,H$\alpha$)
}
\figsetplot{hh460_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.19}
\figsetgrptitle{HH460 ([SII])
}
\figsetplot{hh460_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.20}
\figsetgrptitle{HH476 (g,i,H$\alpha$)
}
\figsetplot{hh476_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.21}
\figsetgrptitle{HH476 ([SII])
}
\figsetplot{hh476_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.22}
\figsetgrptitle{HH477 (g,i,H$\alpha$)
}
\figsetplot{hh477_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.23}
\figsetgrptitle{HH477 ([SII])
}
\figsetplot{hh477_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.24}
\figsetgrptitle{HH478 (g,i,H$\alpha$)
}
\figsetplot{hh478_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.25}
\figsetgrptitle{HH478 ([SII])
}
\figsetplot{hh478_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.26}
\figsetgrptitle{HH721 \& HH724 (g,i,H$\alpha$)
}
\figsetplot{hh721y724_giha.pdf}
\figsetgrpnote{HH721 is in the upper-left; HH724 is below center. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.27}
\figsetgrptitle{HH721 \& HH724 ([SII])
}
\figsetplot{hh721y724_s2.pdf}
\figsetgrpnote{HH721 is in the upper-left; HH724 is below center. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.28}
\figsetgrptitle{HH722 (g,i,H$\alpha$)
}
\figsetplot{hh722_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.29}
\figsetgrptitle{HH722 ([SII])
}
\figsetplot{hh722_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.30}
\figsetgrptitle{HH723 (g,i,H$\alpha$)
}
\figsetplot{hh723_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.31}
\figsetgrptitle{HH723 ([SII])
}
\figsetplot{hh723_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.32}
\figsetgrptitle{HH1278 (g,i,H$\alpha$)
}
\figsetplot{hh1278_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.33}
\figsetgrptitle{HH1278 ([SII])
}
\figsetplot{hh1278_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.34}
\figsetgrptitle{HH1279 (g,i,H$\alpha$)
}
\figsetplot{hh1279_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.35}
\figsetgrptitle{HH1279 ([SII])
}
\figsetplot{hh1279_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.36}
\figsetgrptitle{HH1280 \& HH1281 (g,i,H$\alpha$)
}
\figsetplot{hh1280y1281_giha.pdf}
\figsetgrpnote{HH1280 is near the center; HH1281 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.37}
\figsetgrptitle{HH1280 \& HH1281 ([SII])
}
\figsetplot{hh1280y1281_s2.pdf}
\figsetgrpnote{HH1280 is near the center; HH1281 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.38}
\figsetgrptitle{HH1282 (g,i,H$\alpha$)
}
\figsetplot{hh1282_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.39}
\figsetgrptitle{HH1282 ([SII])
}
\figsetplot{hh1282_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.40}
\figsetgrptitle{HH1283 (g,i,H$\alpha$)
}
\figsetplot{hh1283_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.41}
\figsetgrptitle{HH1283 ([SII])
}
\figsetplot{hh1283_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.42}
\figsetgrptitle{HH1284 (g,i,H$\alpha$)
}
\figsetplot{hh1284_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.43}
\figsetgrptitle{HH1284 ([SII])
}
\figsetplot{hh1284_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.44}
\figsetgrptitle{HH1285 (g,i,H$\alpha$)
}
\figsetplot{hh1285_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.45}
\figsetgrptitle{HH1285 ([SII])
}
\figsetplot{hh1285_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.46}
\figsetgrptitle{HH1286 (g,i,H$\alpha$)
}
\figsetplot{hh1286_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.47}
\figsetgrptitle{HH1286 ([SII])
}
\figsetplot{hh1286_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.48}
\figsetgrptitle{HH1287 (g,i,H$\alpha$)
}
\figsetplot{hh1287_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.49}
\figsetgrptitle{HH1287 ([SII])
}
\figsetplot{hh1287_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.50}
\figsetgrptitle{HH1288 (g,i,H$\alpha$)
}
\figsetplot{hh1288_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.51}
\figsetgrptitle{HH1288 ([SII])
}
\figsetplot{hh1288_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.52}
\figsetgrptitle{HH1289 (g,i,H$\alpha$)
}
\figsetplot{hh1289_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.53}
\figsetgrptitle{HH1289 ([SII])
}
\figsetplot{hh1289_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.54}
\figsetgrptitle{HH1290 (g,i,H$\alpha$)
}
\figsetplot{hh1290_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.55}
\figsetgrptitle{HH1290 ([SII])
}
\figsetplot{hh1290_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.56}
\figsetgrptitle{HH1291 (g,i,H$\alpha$)
}
\figsetplot{hh1291_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.57}
\figsetgrptitle{HH1291 ([SII])
}
\figsetplot{hh1291_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.58}
\figsetgrptitle{HH1292 (g,i,H$\alpha$)
}
\figsetplot{hh1292_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.59}
\figsetgrptitle{HH1292 ([SII])
}
\figsetplot{hh1292_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.60}
\figsetgrptitle{HH1293 (g,i,H$\alpha$)
}
\figsetplot{hh1293_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.61}
\figsetgrptitle{HH1293 ([SII])
}
\figsetplot{hh1293_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.62}
\figsetgrptitle{HH1294 (g,i,H$\alpha$)
}
\figsetplot{hh1294_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.63}
\figsetgrptitle{HH1294 ([SII])
}
\figsetplot{hh1294_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.64}
\figsetgrptitle{HH1295 (g,i,H$\alpha$)
}
\figsetplot{hh1295_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.65}
\figsetgrptitle{HH1295 ([SII])
}
\figsetplot{hh1295_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.66}
\figsetgrptitle{HH1296 (g,i,H$\alpha$)
}
\figsetplot{hh1296_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.67}
\figsetgrptitle{HH1296 ([SII])
}
\figsetplot{hh1296_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.68}
\figsetgrptitle{HH1297 (g,i,H$\alpha$)
}
\figsetplot{hh1297_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.69}
\figsetgrptitle{HH1297 ([SII])
}
\figsetplot{hh1297_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.70}
\figsetgrptitle{HH1298 (g,i,H$\alpha$)
}
\figsetplot{hh1298_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.71}
\figsetgrptitle{HH1298 ([SII])
}
\figsetplot{hh1298_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.72}
\figsetgrptitle{HH1299 (g,i,H$\alpha$)
}
\figsetplot{hh1299_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.73}
\figsetgrptitle{HH1299 ([SII])
}
\figsetplot{hh1299_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.74}
\figsetgrptitle{HH1300 \& HH1302 (g,i,H$\alpha$)
}
\figsetplot{hh1300y1302_giha.pdf}
\figsetgrpnote{HH1300 is to the right of center; HH1302 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.75}
\figsetgrptitle{HH1300 \& HH1302 ([SII])
}
\figsetplot{hh1300y1302_s2.pdf}
\figsetgrpnote{HH1300 is to the right of center; HH1302 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.76}
\figsetgrptitle{HH1301 (g,i,H$\alpha$)
}
\figsetplot{hh1301_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.77}
\figsetgrptitle{HH1301 ([SII])
}
\figsetplot{hh1301_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.78}
\figsetgrptitle{HH1303 (g,i,H$\alpha$)
}
\figsetplot{hh1303_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.79}
\figsetgrptitle{HH1303 ([SII])
}
\figsetplot{hh1303_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.80}
\figsetgrptitle{HH1304 (g,i,H$\alpha$)
}
\figsetplot{hh1304_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.81}
\figsetgrptitle{HH1304 ([SII])
}
\figsetplot{hh1304_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.82}
\figsetgrptitle{HH1305 (g,i,H$\alpha$)
}
\figsetplot{hh1305_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.83}
\figsetgrptitle{HH1305 ([SII])
}
\figsetplot{hh1305_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.84}
\figsetgrptitle{HH1306 (g,i,H$\alpha$)
}
\figsetplot{hh1306_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.85}
\figsetgrptitle{HH1306 ([SII])
}
\figsetplot{hh1306_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.86}
\figsetgrptitle{HH1307 (g,i,H$\alpha$)
}
\figsetplot{hh1307_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.87}
\figsetgrptitle{HH1307 ([SII])
}
\figsetplot{hh1307_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.88}
\figsetgrptitle{HH1308 (g,i,H$\alpha$)
}
\figsetplot{hh1308_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.89}
\figsetgrptitle{HH1308 ([SII])
}
\figsetplot{hh1308_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.90}
\figsetgrptitle{HH1309 (g,i,H$\alpha$)
}
\figsetplot{hh1309_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.91}
\figsetgrptitle{HH1309 ([SII])
}
\figsetplot{hh1309_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.92}
\figsetgrptitle{HH1310 (g,i,H$\alpha$)
}
\figsetplot{hh1310_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.93}
\figsetgrptitle{HH1310 ([SII])
}
\figsetplot{hh1310_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.94}
\figsetgrptitle{HH1311 (g,i,H$\alpha$)
}
\figsetplot{hh1311_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.95}
\figsetgrptitle{HH1311 ([SII])
}
\figsetplot{hh1311_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.96}
\figsetgrptitle{HH1312 (g,i,H$\alpha$)
}
\figsetplot{hh1312_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.97}
\figsetgrptitle{HH1312 ([SII])
}
\figsetplot{hh1312_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.98}
\figsetgrptitle{HH1313 (g,i,H$\alpha$)
}
\figsetplot{hh1313_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.99}
\figsetgrptitle{HH1313 ([SII])
}
\figsetplot{hh1313_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.100}
\figsetgrptitle{HH1314 (g,i,H$\alpha$)
}
\figsetplot{hh1314_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.101}
\figsetgrptitle{HH1314 ([SII])
}
\figsetplot{hh1314_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.102}
\figsetgrptitle{HH1315 (g,i,H$\alpha$)
}
\figsetplot{hh1315_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.103}
\figsetgrptitle{HH1315 ([SII])
}
\figsetplot{hh1315_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.104}
\figsetgrptitle{HH1316 (g,i,H$\alpha$)
}
\figsetplot{hh1316_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.105}
\figsetgrptitle{HH1316 ([SII])
}
\figsetplot{hh1316_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.106}
\figsetgrptitle{HH1317 \& HH1318 (g,i,H$\alpha$)
}
\figsetplot{hh1317y1318_giha.pdf}
\figsetgrpnote{HH1317 is to the right of center; HH1318 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.107}
\figsetgrptitle{HH1317 \& HH1318 ([SII])
}
\figsetplot{hh1317y1318_s2.pdf}
\figsetgrpnote{HH1317 is to the right of center; HH1318 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.108}
\figsetgrptitle{HH1319 (g,i,H$\alpha$)
}
\figsetplot{hh1319_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.109}
\figsetgrptitle{HH1319 ([SII])
}
\figsetplot{hh1319_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.110}
\figsetgrptitle{HH1320 (g,i,H$\alpha$)
}
\figsetplot{hh1320_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.111}
\figsetgrptitle{HH1320 ([SII])
}
\figsetplot{hh1320_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.112}
\figsetgrptitle{HH1321 (g,i,H$\alpha$)
}
\figsetplot{hh1321_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.113}
\figsetgrptitle{HH1321 ([SII])
}
\figsetplot{hh1321_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.114}
\figsetgrptitle{HH1322 (g,i,H$\alpha$)
}
\figsetplot{hh1322_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.115}
\figsetgrptitle{HH1322 ([SII])
}
\figsetplot{hh1322_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.116}
\figsetgrptitle{HH1323 (g,i,H$\alpha$)
}
\figsetplot{hh1323_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.117}
\figsetgrptitle{HH1323 ([SII])
}
\figsetplot{hh1323_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.118}
\figsetgrptitle{HH1324 (g,i,H$\alpha$)
}
\figsetplot{hh1324_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.119}
\figsetgrptitle{HH1324 ([SII])
}
\figsetplot{hh1324_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.120}
\figsetgrptitle{HH1325 (g,i,H$\alpha$)
}
\figsetplot{hh1325_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.121}
\figsetgrptitle{HH1325 ([SII])
}
\figsetplot{hh1325_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.122}
\figsetgrptitle{HH1326 (g,i,H$\alpha$)
}
\figsetplot{hh1326_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.123}
\figsetgrptitle{HH1326 ([SII])
}
\figsetplot{hh1326_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.124}
\figsetgrptitle{HH1327 (g,i,H$\alpha$)
}
\figsetplot{hh1327_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.125}
\figsetgrptitle{HH1327 ([SII])
}
\figsetplot{hh1327_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.126}
\figsetgrptitle{HH1328 (g,i,H$\alpha$)
}
\figsetplot{hh1328_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.127}
\figsetgrptitle{HH1328 ([SII])
}
\figsetplot{hh1328_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.128}
\figsetgrptitle{HH1329 (g,i,H$\alpha$)
}
\figsetplot{hh1329_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.129}
\figsetgrptitle{HH1329 ([SII])
}
\figsetplot{hh1329_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.130}
\figsetgrptitle{HH1330 (g,i,H$\alpha$)
}
\figsetplot{hh1330_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.131}
\figsetgrptitle{HH1330 ([SII])
}
\figsetplot{hh1330_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.132}
\figsetgrptitle{HH1331 (g,i,H$\alpha$)
}
\figsetplot{hh1331_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.133}
\figsetgrptitle{HH1331 ([SII])
}
\figsetplot{hh1331_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.134}
\figsetgrptitle{HH1332 (g,i,H$\alpha$)
}
\figsetplot{hh1332_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.135}
\figsetgrptitle{HH1332 ([SII])
}
\figsetplot{hh1332_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.136}
\figsetgrptitle{HH1333 (g,i,H$\alpha$)
}
\figsetplot{hh1333_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.137}
\figsetgrptitle{HH1333 ([SII])
}
\figsetplot{hh1333_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.138}
\figsetgrptitle{HH1334 (g,i,H$\alpha$)
}
\figsetplot{hh1334_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.139}
\figsetgrptitle{HH1334 ([SII])
}
\figsetplot{hh1334_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.140}
\figsetgrptitle{HH1334A \& HH1334B (g,i,H$\alpha$)
}
\figsetplot{hh1334AB_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.141}
\figsetgrptitle{HH1334A \& HH1334B ([SII])
}
\figsetplot{hh1334AB_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.142}
\figsetgrptitle{HH1335 (g,i,H$\alpha$)
}
\figsetplot{hh1335_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.143}
\figsetgrptitle{HH1335 ([SII])
}
\figsetplot{hh1335_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.144}
\figsetgrptitle{HH1336 (g,i,H$\alpha$)
}
\figsetplot{hh1336_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.145}
\figsetgrptitle{HH1336 ([SII])
}
\figsetplot{hh1336_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.146}
\figsetgrptitle{HH1337 (g,i,H$\alpha$)
}
\figsetplot{hh1337_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.147}
\figsetgrptitle{HH1337 ([SII])
}
\figsetplot{hh1337_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.148}
\figsetgrptitle{HH1338 (g,i,H$\alpha$)
}
\figsetplot{hh1338_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.149}
\figsetgrptitle{HH1338 ([SII])
}
\figsetplot{hh1338_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.150}
\figsetgrptitle{HH1339 (g,i,H$\alpha$)
}
\figsetplot{hh1339_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.151}
\figsetgrptitle{HH1339 ([SII])
}
\figsetplot{hh1339_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.152}
\figsetgrptitle{HH1340 (g,i,H$\alpha$)
}
\figsetplot{hh1340_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.153}
\figsetgrptitle{HH1340 ([SII])
}
\figsetplot{hh1340_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.154}
\figsetgrptitle{HH1341 (g,i,H$\alpha$)
}
\figsetplot{hh1341_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.155}
\figsetgrptitle{HH1341 ([SII])
}
\figsetplot{hh1341_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.156}
\figsetgrptitle{HH1342 (g,i,H$\alpha$)
}
\figsetplot{hh1342_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.157}
\figsetgrptitle{HH1342 ([SII])
}
\figsetplot{hh1342_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.158}
\figsetgrptitle{HH1343 (g,i,H$\alpha$)
}
\figsetplot{hh1343_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.159}
\figsetgrptitle{HH1343 ([SII])
}
\figsetplot{hh1343_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.160}
\figsetgrptitle{HH1344 (g,i,H$\alpha$)
}
\figsetplot{hh1344_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.161}
\figsetgrptitle{HH1344 ([SII])
}
\figsetplot{hh1344_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.162}
\figsetgrptitle{HH1345 (g,i,H$\alpha$)
}
\figsetplot{hh1345_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.163}
\figsetgrptitle{HH1345 ([SII])
}
\figsetplot{hh1345_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.164}
\figsetgrptitle{HH1346 (g,i,H$\alpha$)
}
\figsetplot{hh1346_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.165}
\figsetgrptitle{HH1346 ([SII])
}
\figsetplot{hh1346_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.166}
\figsetgrptitle{HH1347 (g,i,H$\alpha$)
}
\figsetplot{hh1347_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.167}
\figsetgrptitle{HH1347 ([SII])
}
\figsetplot{hh1347_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.168}
\figsetgrptitle{HH1348 (g,i,H$\alpha$)
}
\figsetplot{hh1348_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.169}
\figsetgrptitle{HH1348 ([SII])
}
\figsetplot{hh1348_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.170}
\figsetgrptitle{HH1349 (g,i,H$\alpha$)
}
\figsetplot{hh1349_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.171}
\figsetgrptitle{HH1349 ([SII])
}
\figsetplot{hh1349_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.172}
\figsetgrptitle{HH1350 (g,i,H$\alpha$)
}
\figsetplot{hh1350_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.173}
\figsetgrptitle{HH1350 ([SII])
}
\figsetplot{hh1350_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.174}
\figsetgrptitle{HH1351 \& HH1353 (g,i,H$\alpha$)
}
\figsetplot{hh1351y1353_giha.pdf}
\figsetgrpnote{HH1351 is to the right of center; HH1353 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.175}
\figsetgrptitle{HH1351 \& HH1353 ([SII])
}
\figsetplot{hh1351y1353_s2.pdf}
\figsetgrpnote{HH1351 is to the right of center; HH1353 is to the left. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.176}
\figsetgrptitle{HH1352 (g,i,H$\alpha$)
}
\figsetplot{hh1352_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.177}
\figsetgrptitle{HH1352 ([SII])
}
\figsetplot{hh1352_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.178}
\figsetgrptitle{HH1354 (g,i,H$\alpha$)
}
\figsetplot{hh1354_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.179}
\figsetgrptitle{HH1354 ([SII])
}
\figsetplot{hh1354_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.180}
\figsetgrptitle{HH1355 (g,i,H$\alpha$)
}
\figsetplot{hh1355_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.181}
\figsetgrptitle{HH1355 ([SII])
}
\figsetplot{hh1355_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.182}
\figsetgrptitle{HH1356 (g,i,H$\alpha$)
}
\figsetplot{hh1356_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.183}
\figsetgrptitle{HH1357 (g,i,H$\alpha$)
}
\figsetplot{hh1357_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.184}
\figsetgrptitle{HH1357 ([SII])
}
\figsetplot{hh1357_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.185}
\figsetgrptitle{HH1358 (g,i,H$\alpha$)
}
\figsetplot{hh1358_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.186}
\figsetgrptitle{HH1358 ([SII])
}
\figsetplot{hh1358_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.187}
\figsetgrptitle{HH1359 (g,i,H$\alpha$)
}
\figsetplot{hh1359_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.188}
\figsetgrptitle{HH1359 ([SII])
}
\figsetplot{hh1359_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.189}
\figsetgrptitle{HH1360 (g,i,H$\alpha$)
}
\figsetplot{hh1360_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.190}
\figsetgrptitle{HH1360 ([SII])
}
\figsetplot{hh1360_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.191}
\figsetgrptitle{HH1361 (g,i,H$\alpha$)
}
\figsetplot{hh1361_giha.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.192}
\figsetgrptitle{HH1361 ([SII])}
\figsetplot{hh1361_s2.pdf}
\figsetgrpnote{The HH object is at the center of the image. Each cutout is 462 pixels (2.0\arcmin) on a side; North is up, East is to the left. The color composite image on the left shows H$\alpha$ emission as deep red. The grayscale image on the right shows the [SII] follow-up observations.}
\figsetgrpend

\figsetend

==> hhsummary.tex <==
\startlongtable
\begin{deluxetable*}{lhlll}
\tablecaption{Newly Discovered HH objects\label{tbl:newHH}}
\tablewidth{0pt}
\tablehead{\colhead{HH} & \colhead{} & \colhead{RA(2000)} & \colhead{DEC} & \colhead{Progenitor candidate(s)}}
\startdata
1278 & Aql\_nf26\_A & 18:17:37.7 & -04:40:00 & IRAS 18148-0440 \\
1279 & Aql\_nf08\_A & 18:22:13.7 & -01:58:03 & IRAS 18197-0158 \\ 
1280 & Aql\_nf08\_B & 18:22:22.1 & -01:57:06 & IRAS 18197-0158 \\ 
1281 & Aql\_nf08\_C & 18:22:24.3 & -01:56:54 & IRAS 18197-0158 \\ 
1282 & Aql\_nf26\_B & 18:23:02.2 & -04:58:24 & \nodata \\
1283 & Aql\_nf08\_D & 18:25:14.8 & -02:58:36 & 2MASS J18251133-0258532, 2MASS J18251332-0259549 \\ 
1284 & Aql\_nf01\_G & 18:27:17.8 & -01:59:00 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1285 & Aql\_nf03\_J & 18:28:31.1 & +00:10:03 & Ser-emb 11, Gaia DR3 4272930506004382208 \\ 
1286 & Aql\_nf01\_F & 18:28:41.7 & -01:48:06 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1287 & Aql\_nf03\_H & 18:29:02.6 & +00:12:05 & Ser-emb 11, Gaia DR3 4272930506004382208 \\ 
1288 & Aql\_nf03\_E & 18:29:39.6 & +01:22:56 & IRAS 18269+0116 \\ 
1289 & Aql\_nf01\_E & 18:29:45.0 & -01:37:37 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1290 & Aql\_nf01\_D & 18:29:50.5 & -01:34:55 & IRAS 18264-0143, IRAS 18268-0140 \\ 
107B & Aql\_nf03\_D & 18:29:50.5 & +01:26:52 & IRAS 18269+0116 \\ 
1291 & Aql\_nf01\_C & 18:29:53.1 & -01:29:32 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1292 & Aql\_nf03\_B & 18:29:53.7 & +01:13:18 & Serpens cloud core \\ 
1293 & Aql\_nf03\_C & 18:29:54.0 & +01:10:23 & Serpens cloud core \\ 
%Aql\_nf03 & K & 18:29:55.1 &+00:38:38 \\ 
1294 & Aql\_nf03\_I & 18:30:01.2 & +01:16:21 & Serpens cloud core \\ 
1295 & Aql\_nf01\_A & 18:30:03.0 & -01:36:32 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1296 & Aql\_nf03\_F & 18:30:07.7 & +01:19:52 & Serpens cloud core \\ 
1297 & Aql\_nf01\_B & 18:30:45.3 & -01:21:26 & IRAS 18264-0143, IRAS 18268-0140 \\ 
1298 & Aql\_nf03\_G & 18:32:44.9 & +00:43:16 & Serpens cloud core, IRAS 18301+0035\\ 
1299 & Aql\_nf07\_ D & 18:36:32.8 & -06:43:33 & SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
%Aql\_nf07 & E & 18:36:38.3 & -06:49:07 \\  % DNe
1300 & Aql\_nf06\_C & 18:36:42.7 & -02:19:32 & HGBS J183629.6-022159 \\ 
1301 & Aql\_nf07\_A & 18:36:43.7 & -06:44:28 & SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1302 & Aql\_nf06\_D & 18:36:45.0 & -02:19:15 & HGBS J183629.6-022159 \\ 
1303 & Aql\_nf07\_C & 18:36:46.5 & -06:45:42 & SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1304 & Aql\_nf07\_B & 18:36:48.4 & -06:44:43 & SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1305 & Aql\_nf06\_N & 18:36:53.4 & -01:15:41 & SPICY 87918, SPICY 87939, SPICY 87984 \\ 
%Aql\_nf07 & F & 18:36:57.9 & -06:43:23 \\  % DNe
1306 & Aql\_nf06\_H & 18:38:01.1 & -01:11:25 & {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1307 & Aql\_nf06\_J & 18:38:03.7 & -01:05:00 & {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1308 & Aql\_nf06\_A & 18:38:11.9 & -01:05:07 & {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1309 & Aql\_nf06\_G & 18:38:20.2 & -01:13:45 & {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1310 & Aql\_nf06\_F & 18:38:43.8 & -01:15:37 & {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
% Aql\_nf10 & PN3? & 18:40:47.4 & +00:34:25 \\ PN
1311 & Aql\_nf07\_G & 18:39:09.5 & -07:19:30 & 2MASS J18391236-0720158 \\ 
1312 & Aql\_nf10\_C & 18:40:50.6 & +01:02:03 & IRAS 18383+0059 \\ 
1313 & Aql\_nf10\_D & 18:41:48.5 & +00:52:07 & IRAS 18383+0059 \\ 
1314 & Aql\_nf10\_B & 18:42:00.5 & +01:17:39 & \nodata \\ 
% Aql\_nf10 & PN1? & 18:42:54.6 & +01:22:21 \\ PN
1315 & Aql\_nf10\_G & 18:43:25.4 & +01:06:43 & \nodata \\ 
%Aql\_nf10 & PN2? & 18:45:05.2 & +00:11:58 \\ 
1316 & Aql\_nf10\_H & 18:46:25.8 & +00:28:58 & IRAS 18440+0023 \\ 
1317 & Aql\_nf10\_F & 18:46:32.8 & +00:46:58 & \nodata \\ 
1318 & Aql\_nf10\_E & 18:46:37.1 & +00:46:26 & \nodata \\ 
1319 & Aql\_nf10\_A & 18:46:37.6 & +00:26:12 & IRAS 18440+0023 \\ 
1320 & Aql\_nf11\_B & 18:47:12.1 & +02:14:08 & \nodata \\ 
1321 & Aql\_nf11\_C & 18:47:26.3 & +02:50:58 & IRAS 18454+0250\\ 
% Aql\_nf11 & PN1? & 18:48:58.3 & +02:02:38 \\ PN
1322 & Aql\_nf33\_A & 18:49:38.1 & +00:09:27 & SPICY 92856, 2MASS J18494869+0006072, SPICY 92905, SPICY 92890 \\ 
1323 & Aql\_nf11\_A & 18:50:58.5 & +02:41:37 & IRAS 18484+0237 \\ 
1324 & Aql\_nf33\_D & 18:51:11.8 & +00:24:00 & GGD30IR \citep{2007MNRAS.375..257S}\\ 
% Aql\_nf11 & PN2? & 18:51:25.2 & 03:14:22 \\ PN
1325 & Aql\_nf33\_C & 18:54:44.1 & +00:53:38 & MSX6C G034.0500-00.2977, MSX6C G034.0126-00.2832\\ 
1326 & Aql\_nf12\_E & 18:54:44.7 & +04:02:47 & HIGALBM G036.9422+01.1219 \\ 
1327 & Aql\_nf12\_B & 18:54:45.3 & +04:04:10 & HIGALBM G036.9422+01.1219 \\ 
1328 & Aql\_nf12\_A & 18:54:46.7 & +04:06:34 & HIGALBM G036.9422+01.1219 \\ 
1329 & Aql\_nf12\_D & 18:55:13.4 & +03:59:47 & IRAS 18528+0400 \\ 
1330 & Aql\_nf12\_C & 18:55:19.2 & +04:03:20 & IRAS 18528+0400 \\ 
1331 & Aql\_f03pt5\_S & 18:55:41.7 & +01:12:28 & HIGALBM G034.3721-00.5424 \\ 
1332 & Aql\_f03pt5\_D & 18:55:48.1 &+00:44:18 & AGAL G034.196-00.592, HIGALBM G034.3395-00.6940 \\ 
1333 & Aql\_f03pt5\_R & 18:55:50.0 &+01:08:47 & HIGALBM G034.3721-00.5424 \\ 
1334 & Aql\_f03pt5\_G & 18:56:20.5 &+00:48:45 & HIGALBM G034.3395-00.6940 \\ 
1334A & Aql\_f03pt5\_F & 18:56:21.1 &+00:50:19 & HIGALBM G034.3395-00.6940 \\ 
1334B & Aql\_f03pt5\_E & 18:56:22.6 &+00:50:44 & HIGALBM G034.3395-00.6940 \\ 
1335 & Aql\_f03pt5\_I & 18:56:30.8 &+00:55:13 & HIGALBM G034.3395-00.6940 \\ 
1336 & Aql\_f03pt5\_L & 18:57:22.5 &+01:09:33 & IRAS 18550+0104, IRAS 18555+0056, IRAS 18542+0114 \\ 
1337 & Aql\_f03pt5\_Q & 18:58:15.2 &+01:41:44 & Source in cluster G35.2-0.74N \\ 
1338 & Aql\_f03pt5\_H & 18:58:18.4 &+00:49:30 & IRAS 18566+0048, IRAS 18558+0047 \\ 
1339 & Aql\_f03pt5\_U & 18:58:24.1 &+00:51:20 & IRAS 18566+0048, IRAS 18558+0047 \\ 
1340 & Aql\_f03pt5\_O & 18:58:29.3 &+00:58:30 & IRAS 18566+0048, IRAS 18558+0047 \\ 
1341 & Aql\_f03pt5\_T & 18:58:44.0 &+00:51:39 & IRAS 18566+0048, IRAS 18558+0047 \\ 
% Aql\_f03pt5 & J? & 18:58:52.8 & 02:22:13 \\ Not an HH object
1342 & Aql\_f03pt5\_P & 18:59:03.5 &+00:46:10 & IRAS 18566+0048 \\ 
1343 & Aql\_f03pt5\_C & 18:59:04.3 &+00:44:41 & IRAS 18566+0048 \\ 
1344 & Aql\_f03pt5\_B & 18:59:05.1 &+00:48:30 & IRAS 18566+0048 \\ 
1345 & Aql\_f03pt5\_A & 18:59:09.2 &+00:51:07 & IRAS 18566+0048 \\ 
1346 & Aql\_f03pt5\_N & 18:59:17.6 &+00:58:02 & IRAS 18566+0048 \\ 
1347 & Aql\_f03pt5\_M & 18:59:18.6 &+00:59:39 & IRAS 18566+0048 \\ 
1348 & Aql\_nf13\_J & 19:00:25.7 &+05:20:12 & HIGALBM G038.6940+00.4527, MSX6C G038.8750+00.3088 \\ 
1349 & Aql\_nf13\_E & 19:01:17.6 &+05:11:35 & IRAS 18591+0503, SPICY 96721 \\ 
1350 & Aql\_nf13\_D & 19:01:25.6 &+05:09:02 & IRAS 18591+0503, SPICY 96721 \\
1351 & Aql\_nf13\_A & 19:01:25.9 &+05:14:32 & IRAS 18589+0511 \\ 
1352 & Aql\_nf13\_C & 19:01:28.3 &+05:18:52 & IRAS 18589+0511 \\ 
1353 & Aql\_nf13\_B & 19:01:30.7 &+05:14:35 & IRAS 18589+0511 \\ 
1354 & Aql\_nf13\_I & 19:01:44.7 &+05:21:10 & CORNISH G039.1956+00.2255 \\ 
1354A & Aql\_nf13\_H & 19:01:45.0 &+05:21:59 & CORNISH G039.1956+00.2255 \\ 
1355 & Aql\_nf13\_G & 19:01:48.0 &+05:24:26 & CORNISH G039.1956+00.2255 \\ 
% Aql\_nf13 & SNR? & 19:03:49 & 04:55:48 \\ % Bubble? (2012MNRAS.424.2442S)
1356 & Aql\_f02pt5\_A & 19:07:11.0 &+05:12:28 & HBC 684, IRAS 19045+0518 \\ 
1357 & Aql\_nf23\_F & 19:18:35.4 & +11:41:47 & IRAS 19160+1139, IRAS 19158+1136 \\ 
%Aql\_f01 & E? & 19:20:00.1 & +11:08:30 \\ % IR embedded source, not clear if there is line emission
1358 & Aql\_f01\_A & 19:20:43.8 & +11:04:56 & AS~353 \\ % diffuse nebulosity, possible extension of HH32
1359 & Aql\_f01\_F & 19:20:49.9 & +11:16:00 & Same source as HH~1183-86 \citep{2018ApJ...852...13R} \\ % same as H in Aql\_nf23. embedded in dark cloud
%Aql\_nf23 & H & 19:20:49.9 & +11:16:00 \\ % same as F in Aql\_f01. embedded in dark cloud
1360 & Aql\_f01\_C & 19:21:07.5 & +10:52:20 & IRAS 19190+1048 (HH 250-IRS) \\ % SW of HH250, likely part of same outflow from HH250-IRS
1361 & Aql\_f01\_B & 19:21:21.6 & +10:53:43 & IRAS 19190+1048 (HH 250-IRS) \\ % NE of HH250, likely part of same outflow from HH250-IRS (2019A&A...628A..97C)
\enddata
\tablecomments{Only the first five entries of this table are shown here.  The astrometry for all of the newly discovered HH objects is published in its entirety in machine-readable format.}
\end{deluxetable*}

==> hhsummary_new.tex <==
\startlongtable
\begin{deluxetable*}{lhlllll}
\tablecaption{Newly Discovered HH objects in Ser-Aql\label{tbl:newHH}}
\tablewidth{0pt}
\tablehead{\colhead{HH} & \colhead{} & \colhead{RA(2000)} & \colhead{DEC} & \colhead{$l$} & \colhead{$b$} & \colhead{Progenitor candidate(s)}}
\startdata
1278 & Aql\_nf26\_A & 18:17:37.7 & -04:40:00 &      24.8944 &      5.35275 &
 IRAS 18148-0440 \\
1279 & Aql\_nf08\_A & 18:22:13.7 & -01:58:03 &      27.8314 &      5.58965 &
 IRAS 18197-0158 \\ 
1280 & Aql\_nf08\_B & 18:22:22.1 & -01:57:06 &      27.8617 &      5.56593 &
 IRAS 18197-0158 \\ 
1281 & Aql\_nf08\_C & 18:22:24.3 & -01:56:54 &      27.8689 &      5.55934 &
 IRAS 18197-0158 \\ 
1282 & Aql\_nf26\_B & 18:23:02.2 & -04:58:24 &      25.2522 &      4.01779 &
 \nodata \\
1283 & Aql\_nf08\_D & 18:25:14.8 & -02:58:36 &      27.2825 &      4.45485 &
 2MASS J18251133-0258532, 2MASS J18251332-0259549 \\ 
1284 & Aql\_nf01\_G & 18:27:17.8 & -01:59:00 &      28.4034 &      4.45864 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1285 & Aql\_nf03\_J & 18:28:31.1 & 00:10:03 &      30.4617 &      5.17454 &
 Ser-emb 11, Gaia DR3 4272930506004382208 \\ 
1286 & Aql\_nf01\_F & 18:28:41.7 & -01:48:06 &      28.7264 &      4.23200 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1287 & Aql\_nf03\_H & 18:29:02.6 & 00:12:05 &      30.5523 &      5.07334 &
 Ser-emb 11, Gaia DR3 4272930506004382208 \\ 
1288 & Aql\_nf03\_E & 18:29:39.6 & 01:22:56 &      31.6779 &      5.47548 &
 IRAS 18269+0116 \\ 
1289 & Aql\_nf01\_E & 18:29:45.0 & -01:37:37 &      29.0034 &      4.07815 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1290 & Aql\_nf01\_D & 18:29:50.5 & -01:34:55 &      29.0540 &      4.07847 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
107B & Aql\_nf03\_D & 18:29:50.5 & 01:26:52 &      31.7573 &      5.46495 &
 IRAS 18269+0116 \\ 
1291 & Aql\_nf01\_C & 18:29:53.1 & -01:29:32 &      29.1389 &      4.11006 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1292 & Aql\_nf03\_B & 18:29:53.7 & 01:13:18 &      31.5613 &      5.35000 &
 Serpens cloud core \\ 
1293 & Aql\_nf03\_C & 18:29:54.0 & 01:10:23 &      31.5184 &      5.32671 &
 Serpens cloud core \\ 
1294 & Aql\_nf03\_I & 18:30:01.2 & 01:16:21 &      31.6211 &      5.34537 &
 Serpens cloud core \\ 
1295 & Aql\_nf01\_A & 18:30:03.0 & -01:36:32 &      29.0540 &      4.01985 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1296 & Aql\_nf03\_F & 18:30:07.7 & 01:19:52 &      31.6859 &      5.34800 &
 Serpens cloud core \\ 
1297 & Aql\_nf01\_B & 18:30:45.3 & -01:21:26 &      29.3592 &      3.97885 &
 IRAS 18264-0143, IRAS 18268-0140 \\ 
1298 & Aql\_nf03\_G & 18:32:44.9 & 00:43:16 &      31.4409 &      4.48695 &
 Serpens cloud core, IRAS 18301+0035\\ 
1299 & Aql\_nf07\_ D & 18:36:32.8 & -06:43:33 &      25.2520 &     0.228420 &
 SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1300 & Aql\_nf06\_C & 18:36:42.7 & -02:19:32 &      29.1810 &      2.21213 &
 HGBS J183629.6-022159 \\ 
1301 & Aql\_nf07\_A & 18:36:43.7 & -06:44:28 &      25.2591 &     0.181341 &
 SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1302 & Aql\_nf06\_D & 18:36:45.0 & -02:19:15 &      29.1896 &      2.20579 &
 HGBS J183629.6-022159 \\ 
1303 & Aql\_nf07\_C & 18:36:46.5 & -06:45:42 &      25.2462 &     0.161605 &
 SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1304 & Aql\_nf07\_B & 18:36:48.4 & -06:44:43 &      25.2644 &     0.162153 &
 SSTGLMC G025.2255+00.2884, IRAS 18327-0645 \\ 
1305 & Aql\_nf06\_N & 18:36:53.4 & -01:15:41 &      30.1483 &      2.65985 &
 SPICY 87918, SPICY 87939, SPICY 87984 \\ 
1306 & Aql\_nf06\_H & 18:38:01.1 & -01:11:25 &      30.3408 &      2.44161 &
 {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1307 & Aql\_nf06\_J & 18:38:03.7 & -01:05:00 &      30.4409 &      2.48089 &
 {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1308 & Aql\_nf06\_A & 18:38:11.9 & -01:05:07 &      30.4549 &      2.44962 &
 {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1309 & Aql\_nf06\_G & 18:38:20.2 & -01:13:45 &      30.3426 &      2.35307 &
 {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1310 & Aql\_nf06\_F & 18:38:43.8 & -01:15:37 &      30.3599 &      2.25142 &
 {IRAS 18358-0112}, see also \citep{2021ApJS..254...33K} \\ 
1311 & Aql\_nf07\_G & 18:39:09.5 & -07:19:30 &      25.0171 &    -0.622316 &
 2MASS J18391236-0720158 \\ 
1312 & Aql\_nf10\_C & 18:40:50.6 & 01:02:03 &      32.6447 &      2.82884 &
 IRAS 18383+0059 \\ 
1313 & Aql\_nf10\_D & 18:41:48.5 & 00:52:07 &      32.6073 &      2.53868 &
 IRAS 18383+0059 \\ 
1314 & Aql\_nf10\_B & 18:42:00.5 & 01:17:39 &      33.0093 &      2.68810 &
 \nodata \\ 
1315 & Aql\_nf10\_G & 18:43:25.4 & 01:06:43 &      33.0082 &      2.29025 &
 \nodata \\ 
1316 & Aql\_nf10\_H & 18:46:25.8 & 00:28:58 &      32.7907 &      1.33449 &
 IRAS 18440+0023 \\ 
1317 & Aql\_nf10\_F & 18:46:32.8 & 00:46:58 &      33.0711 &      1.44530 &
 \nodata \\ 
1318 & Aql\_nf10\_E & 18:46:37.1 & 00:46:26 &      33.0713 &      1.42530 &
 \nodata \\ 
1319 & Aql\_nf10\_A & 18:46:37.6 & 00:26:12 &      32.7720 &      1.26971 &
 IRAS 18440+0023 \\ 
1320 & Aql\_nf11\_B & 18:47:12.1 & 02:14:08 &      34.4395 &      1.96140 &
 \nodata \\ 
1321 & Aql\_nf11\_C & 18:47:26.3 & 02:50:58 &      35.0134 &      2.18817 &
 IRAS 18454+0250\\ 
1322 & Aql\_nf33\_A & 18:49:38.1 & 00:09:27 &      32.8665 &     0.473079 &
 SPICY 92856, 2MASS J18494869+0006072, SPICY 92905, SPICY 92890 \\ 
1323 & Aql\_nf11\_A & 18:50:58.5 & 02:41:37 &      35.2768 &      1.33091 &
 IRAS 18484+0237 \\ 
1324 & Aql\_nf33\_D & 18:51:11.8 & 00:24:00 &      33.2604 &     0.236187 &
 GGD30IR \citep{2007MNRAS.375..257S}\\ 
1325 & Aql\_nf33\_C & 18:54:44.1 & 00:53:38 &      34.1033 &    -0.325777 &
 MSX6C G034.0500-00.2977, MSX6C G034.0126-00.2832\\ 
1326 & Aql\_nf12\_E & 18:54:44.7 & 04:02:47 &      36.9101 &      1.10979 &
 HIGALBM G036.9422+01.1219 \\ 
1327 & Aql\_nf12\_B & 18:54:45.3 & 04:04:10 &      36.9318 &      1.11808 &
 HIGALBM G036.9422+01.1219 \\ 
1328 & Aql\_nf12\_A & 18:54:46.7 & 04:06:34 &      36.9700 &      1.13113 &
 HIGALBM G036.9422+01.1219 \\ 
1329 & Aql\_nf12\_D & 18:55:13.4 & 03:59:47 &      36.9200 &     0.980824 &
 IRAS 18528+0400 \\ 
1330 & Aql\_nf12\_C & 18:55:19.2 & 04:03:20 &      36.9836 &     0.986347 &
 IRAS 18528+0400 \\ 
1331 & Aql\_f03pt5\_S & 18:55:41.7 & 01:12:28 &      34.4921 &    -0.396121 &
 HIGALBM G034.3721-00.5424 \\ 
1332 & Aql\_f03pt5\_D & 18:55:48.1 & 00:44:18 &      34.0865 &    -0.634017 &
 AGAL G034.196-00.592, HIGALBM G034.3395-00.6940 \\ 
1333 & Aql\_f03pt5\_R & 18:55:50.0 & 01:08:47 &      34.4532 &    -0.454897 &
 HIGALBM G034.3721-00.5424 \\ 
1334 & Aql\_f03pt5\_G & 18:56:20.5 & 00:48:45 &      34.2141 &    -0.720302 &
 HIGALBM G034.3395-00.6940 \\ 
1334A & Aql\_f03pt5\_F & 18:56:21.1 & 00:50:19 &      34.2384 &    -0.710613 &
 HIGALBM G034.3395-00.6940 \\ 
1334B & Aql\_f03pt5\_E & 18:56:22.6 & 00:50:44 &      34.2475 &    -0.713006 &
 HIGALBM G034.3395-00.6940 \\ 
1335 & Aql\_f03pt5\_I & 18:56:30.8 & 00:55:13 &      34.3296 &    -0.709312 &
 HIGALBM G034.3395-00.6940 \\ 
1336 & Aql\_f03pt5\_L & 18:57:22.5 & 01:09:33 &      34.6404 &    -0.791946 &
 IRAS 18550+0104, IRAS 18555+0056, IRAS 18542+0114 \\ 
1337 & Aql\_f03pt5\_Q & 18:58:15.2 & 01:41:44 &      35.2179 &    -0.742390 &
 Source in cluster G35.2-0.74N \\ 
1338 & Aql\_f03pt5\_H & 18:58:18.4 & 00:49:30 &      34.4494 &     -1.15167 &
 IRAS 18566+0048, IRAS 18558+0047 \\ 
1339 & Aql\_f03pt5\_U & 18:58:24.1 & 00:51:20 &      34.4874 &     -1.15886 &
 IRAS 18566+0048, IRAS 18558+0047 \\ 
1340 & Aql\_f03pt5\_O & 18:58:29.3 & 00:58:30 &      34.6036 &     -1.12361 &
 IRAS 18566+0048, IRAS 18558+0047 \\ 
1341 & Aql\_f03pt5\_T & 18:58:44.0 & 00:51:39 &      34.5300 &     -1.23021 &
 IRAS 18566+0048, IRAS 18558+0047 \\ 
1342 & Aql\_f03pt5\_P & 18:59:03.5 & 00:46:10 &      34.4857 &     -1.34421 &
 IRAS 18566+0048 \\ 
1343 & Aql\_f03pt5\_C & 18:59:04.3 & 00:44:41 &      34.4652 &     -1.35847 &
 IRAS 18566+0048 \\ 
1344 & Aql\_f03pt5\_B & 18:59:05.1 & 00:48:30 &      34.5234 &     -1.33239 &
 IRAS 18566+0048 \\ 
1345 & Aql\_f03pt5\_A & 18:59:09.2 & 00:51:07 &      34.5700 &     -1.32768 &
 IRAS 18566+0048 \\ 
1346 & Aql\_f03pt5\_N & 18:59:17.6 & 00:58:02 &      34.6886 &     -1.30619 &
 IRAS 18566+0048 \\ 
1347 & Aql\_f03pt5\_M & 18:59:18.6 & 00:59:39 &      34.7144 &     -1.29760 &
 IRAS 18566+0048 \\ 
1348 & Aql\_nf13\_J & 19:00:25.7 & 05:20:12 &      38.7047 &     0.438885 &
 HIGALBM G038.6940+00.4527, MSX6C G038.8750+00.3088 \\ 
1349 & Aql\_nf13\_E & 19:01:17.6 & 05:11:35 &      38.6755 &     0.181705 &
 IRAS 18591+0503, SPICY 96721 \\ 
1350 & Aql\_nf13\_D & 19:01:25.6 & 05:09:02 &      38.6529 &     0.132739 &
 IRAS 18591+0503, SPICY 96721 \\
1351 & Aql\_nf13\_A & 19:01:25.9 & 05:14:32 &      38.7349 &     0.173581 &
 IRAS 18589+0511 \\ 
1352 & Aql\_nf13\_C & 19:01:28.3 & 05:18:52 &      38.8037 &     0.197779 &
 IRAS 18589+0511 \\ 
1353 & Aql\_nf13\_B & 19:01:30.7 & 05:14:35 &      38.7448 &     0.156254 &
 IRAS 18589+0511 \\ 
1354 & Aql\_nf13\_I & 19:01:44.7 & 05:21:10 &      38.8689 &     0.154830 &
 CORNISH G039.1956+00.2255 \\ 
1354A & Aql\_nf13\_H & 19:01:45.0 & 05:21:59 &      38.8816 &     0.159954 &
 CORNISH G039.1956+00.2255 \\ 
1355 & Aql\_nf13\_G & 19:01:48.0 & 05:24:26 &      38.9236 &     0.167580 &
 CORNISH G039.1956+00.2255 \\ 
1356 & Aql\_f02pt5\_A & 19:07:11.0 & 05:12:28 &      39.3611 &     -1.11466 &
 HBC 684, IRAS 19045+0518 \\ 
1357 & Aql\_nf23\_F & 19:18:35.4 & 11:41:47 &      46.4182 &    -0.605468 &
 IRAS 19160+1139, IRAS 19158+1136 \\ 
1358 & Aql\_f01\_A & 19:20:43.8 & 11:04:56 &      46.1214 &     -1.35660 &
 AS~353 \\ % diffuse nebulosity, possible extension of HH32
1359 & Aql\_f01\_F & 19:20:49.9 & 11:16:00 &      46.2960 &     -1.29202 &
 Same source as HH~1183-86 \citep{2018ApJ...852...13R} \\ % same as H in Aql\_nf23. embedded in dark cloud
1360 & Aql\_f01\_C & 19:21:07.5 & 10:52:20 &      45.9814 &     -1.54080 &
 IRAS 19190+1048 (HH 250-IRS) \\ % SW of HH250, likely part of same outflow from HH250-IRS
1361 & Aql\_f01\_B & 19:21:21.6 & 10:53:43 &      46.0289 &     -1.58090 &
 IRAS 19190+1048 (HH 250-IRS) \\ % NE of HH250, likely part of same outflow from HH250-IRS (2019A
\enddata
\tablecomments{Only the first five entries of this table are shown here.  The astrometry for all of the newly discovered HH objects is published in its entirety in machine-readable format.}
\end{deluxetable*}

==> previoushh.tex <==
\startlongtable
\begin{deluxetable*}{lllll}
\tablecaption{Previously Discovered HH objects in Ser-Aql\label{tbl:oldHH}}
\tablewidth{0pt}
\tablehead{\colhead{HH} & \colhead{RA(J2000)} & \colhead{DEC} & \colhead{Progenitor candidate(s)}}
\startdata
%Aql\_nf26 & 18:17:37.7 & -04:40:00 & IRAS 18148-0440 \\
32 & 19:20:30.0 & +11:02:00 & AS353A, B, or C \\
106 & 18:29:18.8 & +01:14:17 & Gaia DR3 4273733394303463936 \\
107 & 18:29:48.0 & +01:25:55 & Gaia DR3 4273733394303463936 \\
108 & 18:35:36.2 & -00:35:09 & IRAS 18331-0035 \\
109 & 18:35:39.0 & -00:34:20 & IRAS 18331-0035 \\
172 & 18:54:05.9 & +00:32:41 &  Not seen in our images \\
%221 & 19:29:00.9 & +09:38:43 & Gaia DR3 4308446999329032064 \\
250 & 19:21:13.7 & +10 52 31 & IRAS 19190+1048 (HH 250-IRS) \\
332 & 19:20:26.8 & +11:00:38 & AS353A, B, or C \\
455 & 18:30:22.8 & +01:16:19 & Ser-emb 24, 29 \\
456 & 18:29:59.3 & +01:11:15 & Star, not HH object \\
457 & 18:29:59.9 & +01:10:46 & Not seen in our images \\
458 & 18:29:58.1 & +01:13:43 & IRAS 18273+0113? \\
459 & 18:30:02.7 & +01:14:45 & Serpens embedded source \\
460 & 18:29:38.7 & +01:18:24 & IRAS 18273+0113? \\
476 & 18:28:59.5 & +00:29:13 & Ser-emb 17? \\
477 & 18:29:38.3 & +01:20:24 & Gaia DR3 4273733394303463936 \\
478 & 18:29:56.5 & +01:15:40 & Gaia DR3 4273721849431352960 \\
721 & 18:51:44.0 & +00:29:16 & [GE91] GGD 30 I1 \\
722 & 18:51:26.2 & +00:29:04 & [GE91] GGD 30 I1 \\
723 & 18:51:32.0 & +00:28:47 & [GE91] GGD 30 I1 \\
724 & 18:51:42.8 & +00:28:31 & [GE91] GGD 30 I1 \\
1183 & 19:20:24.8 & +11:20:10 & HH1183–1186 IRS1-8\tablenotemark{a} \\
1184 & 19:20:25.1 & +11:19:54 & HH1183–1186 IRS1-8 \\
1185 & 19:20:28.7 & +11:19:24 & HH1183–1186 IRS1-8 \\
1186 & 19:20:29.5 & +11:19:43 & HH1183–1186 IRS1-8 \\
1187 & 19:20:11.9 & +11:00:40 & AS353A, B, or C \\
1188 & 19:20:21.3 & +11:01:16 & AS353A, B, or C \\
1189 & 19:20:24.5 & +11:01:28 & AS353A, B, or C \\
1190 & 19:21:10.9 & +11:03:50 & AS353A, B, or C \\
1191 & 19:21:13.2 & +11:04:01 & AS353A, B, or C \\
1192 & 19:21:26.0 & +11:19:23 & SSTc2d J192134.8+112123  \\
1193 & 19:21:42.6 & +11:22:41 & SSTc2d J192134.8+112123  \\
1194 & 19:21:43.7 & +11:22:51 & SSTc2d J192134.8+112123  \\
\enddata
\tablecomments{Only the first five entries of this table are shown here.  The astrometry for all of the newly discovered HH objects is published in its entirety in machine-readable format.}
\tablenotetext{a}{The properties of these progenitor candidates are given in \citet{2018ApJ...852...13R}.}
\end{deluxetable*}

%HH~106-109 discovered by \citet{1992A&A...256L...1R}.
%HH~455,458-460,476-478 discovered by \citet{1999A&A...347..565Z}.
%HH~455-460 discovered by \citet{1999MNRAS.309..141D}.



==> previoushh_new.tex <==
\startlongtable
\begin{deluxetable*}{lllllll}
\tablecaption{Previously Discovered HH objects in Ser-Aql\label{tbl:oldHH}}
\tablewidth{0pt}
\tablehead{\colhead{HH} & \colhead{RA(2000)} & \colhead{DEC} & \colhead{$l$} & \colhead{$b$} & \colhead{Progenitor candidate(s)}}
\startdata
32 & 19:20:30.0 & +11:02:00 &      46.0517 &     -1.32971 & AS353A, B, or C \\
106 & 18:29:18.8 & +01:14:17 &      31.5094 &      5.48685 &
 Gaia DR3 4273733394303463936 \\
107 & 18:29:48.0 & +01:25:55 &      31.7384 &      5.46700 &
 Gaia DR3 4273733394303463936 \\
108 & 18:35:36.2 & -00:35:09 &      31.6468 &      3.79017 & IRAS 18331-0035 \\
109 & 18:35:39.0 & -00:34:20 &      31.6400 &      3.77358 & IRAS 18331-0035 \\
172 & 18:54:05.9 & +00:32:41 &      33.7199 &    -0.343397 &
 Not seen in our images \\
%221 & 19:29:00.9 & +09:38:43 &      45.9961 &     -1.56176 &
% Gaia DR3 4308446999329032064 \\
250 & 19:21:13.7 & +10:52:31 &      46.0254 &     -1.32884 &
 IRAS 19190+1048 (HH 250-IRS) \\
332 & 19:20:26.8 & +11:00:38 &      31.6618 &      5.26504 & AS353A, B, or C \\
455 & 18:30:22.8 & +01:16:19 &      31.5415 &      5.31365 & Ser-emb 24, 29 \\
456 & 18:29:59.3 & +01:11:15 &      31.5354 &      5.30775 &
 Star, not HH object \\
457 & 18:29:59.9 & +01:10:46 &      31.5759 &      5.33685 &
 Not seen in our images \\
458 & 18:29:58.1 & +01:13:43 &      31.6001 &      5.32765 & IRAS 18273+0113? \\
459 & 18:30:02.7 & +01:14:45 &      31.6087 &      5.44437 &
 Serpens embedded source \\
460 & 18:29:38.7 & +01:18:24 &      30.8013 &      5.21541 & IRAS 18273+0113? \\
476 & 18:28:59.5 & +00:29:13 &      31.6377 &      5.46105 & Ser-emb 17? \\
477 & 18:29:38.3 & +01:20:24 &      31.6019 &      5.35760 &
 Gaia DR3 4273733394303463936 \\
478 & 18:29:56.5 & +01:15:40 &      33.3997 &     0.156808 &
 Gaia DR3 4273721849431352960 \\
721 & 18:51:44.0 & +00:29:16 &      33.3629 &     0.221293 & [GE91] GGD 30 I1 \\
722 & 18:51:26.2 & +00:29:04 &      33.3697 &     0.197633 & [GE91] GGD 30 I1 \\
723 & 18:51:32.0 & +00:28:47 &      33.3863 &     0.155558 & [GE91] GGD 30 I1 \\
724 & 18:51:42.8 & +00:28:31 &      46.3092 &     -1.16887 & [GE91] GGD 30 I1 \\
1183 & 19:20:24.8 & +11:20:10 &      46.3058 &     -1.17204 &
 HH1183–1186 IRS1-8\tablenotemark{a} \\
1184 & 19:20:25.1 & +11:19:54 &      46.3054 &     -1.18894 &
 HH1183–1186 IRS1-8 \\
1185 & 19:20:28.7 & +11:19:24 &      46.3116 &     -1.18935 &
 HH1183–1186 IRS1-8 \\
1186 & 19:20:29.5 & +11:19:43 &      45.9973 &     -1.27476 &
 HH1183–1186 IRS1-8 \\
1187 & 19:20:11.9 & +11:00:40 &      46.0242 &     -1.30403 & AS353A, B, or C \\
1188 & 19:20:21.3 & +11:01:16 &      46.0333 &     -1.31402 & AS353A, B, or C \\
1189 & 19:20:24.5 & +11:01:28 &      46.1572 &     -1.46305 & AS353A, B, or C \\
1190 & 19:21:10.9 & +11:03:50 &      46.1644 &     -1.46991 & AS353A, B, or C \\
1191 & 19:21:13.2 & +11:04:01 &      46.4151 &     -1.39574 & AS353A, B, or C \\
1192 & 19:21:26.0 & +11:19:23 &      46.4955 &     -1.42973 &
 SSTc2d J192134.8+112123 \\
1193 & 19:21:42.6 & +11:22:41 &      46.5001 &     -1.43239 &
 SSTc2d J192134.8+112123 \\
\enddata
\tablecomments{Only the first five entries of this table are shown here.  The astrometry for all of the newly discovered HH objects is published in its entirety in machine-readable format.}
\tablenotetext{a}{The properties of these progenitor candidates are given in \citet{2018ApJ...852...13R}.}
\end{deluxetable*}

%HH~106-109 discovered by \citet{1992A&A...256L...1R}.
%HH~455,458-460,476-478 discovered by \citet{1999A&A...347..565Z}.
%HH~455-460 discovered by \citet{1999MNRAS.309..141D}.

==> progenitors.tex <==
\startlongtable
\begin{deluxetable*}{lllllll}
\tablecolumns{7}
\tablewidth{0pt}
\tablecaption{\label{tbl:progens} Progenitor candidates and their distances, either from Gaia, the \citet{Edenhofer24} dust maps, or a maser-based parallax in the case of G35.2-0.74N \citep{Zhang09}.}
\tablehead{\colhead{Stars} & \colhead{RA (J2000)} & \colhead{Dec} & \colhead{d} & \colhead{$\sigma_d^-$} & \colhead{$\sigma_d^+$} & \colhead{d src}}
\startdata
IRAS 18148-0440 & 274.3748 & -4.6609 & 241 & 25 & 13 & dust \\
IRAS 18197-0158 & 275.5929 & -1.9498 & 475 & 18 & 40 & dust \\
2MASS J18251133-0258532 & 276.2972 & -2.9815 & 255 & 9 & 13 & dust \\
2MASS J18251332-0259549 & 276.3055 & -2.9986 & 255 & 9 & 13 & dust \\
IRAS 18264-0143 & 277.272 & -1.6991 & 469 & 25 & 14 & dust \\
IRAS 18268-0140 & 277.3475 & -1.6488 & 469 & 25 & 14 & dust \\
Ser-emb 7 & 277.2252 & 0.4916 & 444 & 55 & 11 & dust \\
MMS 1 & 277.4575 & 1.2557 & 443 & 59 & 13 & dust \\
IRAS 18269+0116 & 277.3832 & 1.3118 & 442 & 28 & 28 & Gaia \\
Serpens Cloud Core & 277.4542 & 1.2467 & 443 & 59 & 13 & dust \\
IRAS 18301+0035 & 278.1631 & 0.6313 & 492 & 22 & 49 & dust \\
IRAS 18327-0645 & 278.8514 & -6.7165 & 252 & 7 & 8 & dust \\
SSTGLMC G025.2255+00.2884 & 279.0706 & -6.7218 & 252 & 7 & 8 & dust \\
HGBS J183629.6-022159 & 279.1235 & -2.3666 & 479 & 15 & 22 & dust \\
SPICY 87984 & 279.193 & -1.1749 & 484 & 11 & 21 & dust \\
SPICY 87939 & 279.1691 & -1.2015 & 484 & 11 & 21 & dust \\
SPICY 87918 & 279.1619 & -1.2247 & 484 & 11 & 21 & dust \\
IRAS 18358-0112 & 279.6079 & -1.1642 & 482 & 12 & 16 & dust \\
2MASS J18391236-0720158 & 279.8015 & -7.3377 & 252 & 10 & 10 & dust \\
IRAS 18383+0059 & 280.2154 & 1.0358 & 489 & 13 & 13 & dust \\
IRAS 18440+0023 & 281.6343 & 0.4524 & 623 & 43 & 33 & dust \\
IRAS 18454+0250 & 282.0028 & 2.9048 & 610 & 66 & 72 & dust \\
SPICY 92856 & 282.4536 & 0.1079 & 628 & 22 & 22 & dust \\
2MASS J18494869+0006072 & 282.4529 & 0.102 & 628 & 22 & 22 & dust \\
SPICY 92905 & 282.4845 & 0.1893 & 627 & 24 & 26 & dust \\
SPICY 92890 & 282.4712 & 0.2159 & 627 & 24 & 26 & dust \\
IRAS 18484+0237 & 282.7392 & 2.6811 & 583 & 86 & 43 & dust \\
GGD30IR & 282.9188 & 0.4828 & 611 & 42 & 20 & dust \\
MSX6C G034.0126-00.2832 & 283.6346 & 0.8594 & 606 & 16 & 20 & dust \\
MSX6C G034.0500-00.2977 & 283.6346 & 0.8594 & 606 & 16 & 20 & dust \\
HIGALBM G036.9422+01.1219 & 283.6902 & 4.0805 & 547 & 18 & 13 & dust \\
IRAS 18528+0400 & 283.8458 & 4.0764 & 570 & 35 & 35 & Gaia \\
HIGALBM G034.3721-00.5424 & 283.9992 & 1.0342 & 603 & 20 & 23 & dust \\
AGAL G034.196-00.592 & 283.9632 & 0.8555 & 606 & 16 & 22 & dust \\
HIGALBM G034.3395-00.6940 & 284.1192 & 0.9361 & 606 & 16 & 25 & dust \\
IRAS 18555+0056 & 284.5353 & 1.0116 & 605 & 21 & 23 & dust \\
IRAS 18550+0104 & 284.4038 & 1.1356 & 606 & 19 & 27 & dust \\
IRAS 18542+0114 & 284.2011 & 1.3131 & 588 & 31 & 15 & dust \\
{[BCM2016]}~8a/G35.2-0.74N & 284.5543 & 1.6767 & 2190 & 200 & 240 & maser \\
IRAS 18558+0047 & 284.5999 & 0.8649 & 605 & 21 & 20 & dust \\
IRAS 18566+0048 & 284.8058 & 0.8775 & 606 & 24 & 20 & dust \\
HIGALBM G038.6940+00.4527 & 285.0898 & 5.3335 & 686 & 52 & 30 & dust \\
MSX6C G038.8750+00.3088 & 285.3017 & 5.4286 & 688 & 50 & 25 & dust \\
IRAS 18591+0503 & 285.3962 & 5.1303 & 690 & 40 & 27 & dust \\
IRAS 18589+0511 & 285.3606 & 5.2574 & 690 & 44 & 28 & dust \\
CORNISH G039.1956+00.2255 & 285.5232 & 5.6755 & 686 & 56 & 24 & dust \\
HBC 684 & 286.7911 & 5.2197 & 696 & 35 & 23 & dust \\
IRAS 19045+0518 & 286.7488 & 5.382 & 699 & 54 & 27 & dust \\
IRAS 19160+1139 & 289.6078 & 11.7472 & 404 & 9 & 11 & dust \\
IRAS 19158+1136 & 289.5513 & 11.6981 & 404 & 8 & 10 & dust \\
AS 353 & 290.1291 & 11.0318 & 395 & 3 & 3 & Gaia \\
IRAS 19190+1048 & 290.3443 & 10.8992 & 405 & 5 & 7 & dust \\
IRAS 18331-0035 & 278.9253 & -0.5557 & 484 & 15 & 20 & dust \\
Ser-emb 8 & 277.4504 & 1.2792 & 443 & 57 & 13 & dust \\
IRAS 18273+0113 & 277.4568 & 1.2561 & 443 & 59 & 13 & dust \\
Ser-emb 17 & 277.2758 & 0.512 & 444 & 55 & 11 & dust \\
2MASS J18300341+0116191 & 277.5142 & 1.2719 & 443 & 11 & 11 & Gaia \\
HH1183–1186 IRS1 & 290.1075 & 11.3331 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS2 & 290.1077 & 11.3316 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS3 & 290.1082 & 11.3356 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS4 & 290.1085 & 11.3312 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS5 & 290.109 & 11.3303 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS6 & 290.1113 & 11.3321 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS7 & 290.1127 & 11.3365 & 405 & 6 & 7 & dust \\
HH1183–1186 IRS8 & 290.1138 & 11.3323 & 405 & 6 & 7 & dust \\
SSTc2d J192134.8+112123 & 290.3951 & 11.3565 & 405 & 6 & 7 & dust \\
\enddata
\end{deluxetable*}

==> progenitors_new.tex <==
\startlongtable
\begin{deluxetable*}{lllllllll}
\tablecolumns{7}
\tablewidth{0pt}
\tablecaption{\label{tbl:progens} Progenitor Candidates and Their Distances}
\tablehead{\colhead{Stars} & \colhead{RA (2000)} & \colhead{Dec} & \colhead{$l$} & \colhead{$b$} & \colhead{d (pc)} & \colhead{$\sigma_d^-$} & \colhead{$\sigma_d^+$} & \colhead{d src\tablenotemark{a}}}
\startdata
IRAS 18148-0440 & 274.3748 & -4.6609 &      24.8944 &      5.35275 & 241  & 25 
 & 13  & dust \\
IRAS 18197-0158 & 275.5929 & -1.9498 &      27.8314 &      5.58965 & 475  & 18 
 & 40  & dust \\
2MASS J18251133-0258532 & 276.2972 & -2.9815 &      27.8617 &      5.56593 &
 255  & 9  & 13  & dust \\
2MASS J18251332-0259549 & 276.3055 & -2.9986 &      27.8689 &      5.55934 &
 255  & 9  & 13  & dust \\
IRAS 18264-0143 & 277.272 & -1.6991 &      25.2522 &      4.01779 & 469  & 25  &
 14  & dust \\
IRAS 18268-0140 & 277.3475 & -1.6488 &      27.2825 &      4.45485 & 469  & 25 
 & 14  & dust \\
Ser-emb 7 & 277.2252 & 0.4916 &      28.4034 &      4.45864 & 444  & 55  & 11  &
 dust \\
MMS 1 & 277.4575 & 1.2557 &      30.4617 &      5.17454 & 443  & 59  & 13  &
 dust \\
IRAS 18269+0116 & 277.3832 & 1.3118 &      28.7264 &      4.23200 & 442  & 28  &
 28  & Gaia \\
Serpens Cloud Core & 277.4542 & 1.2467 &      30.5523 &      5.07334 & 443  &
 59  & 13  & dust \\
IRAS 18301+0035 & 278.1631 & 0.6313 &      31.6779 &      5.47548 & 492  & 22  &
 49  & dust \\
IRAS 18327-0645 & 278.8514 & -6.7165 &      29.0034 &      4.07815 & 252  & 7  &
 8  & dust \\
SSTGLMC G025.2255+00.2884 & 279.0706 & -6.7218 &      29.0540 &      4.07847 &
 252  & 7  & 8  & dust \\
HGBS J183629.6-022159 & 279.1235 & -2.3666 &      31.7573 &      5.46495 & 479 
 & 15  & 22  & dust \\
SPICY 87984 & 279.193 & -1.1749 &      29.1389 &      4.11006 & 484  & 11  & 21 
 & dust \\
SPICY 87939 & 279.1691 & -1.2015 &      31.5613 &      5.35000 & 484  & 11  &
 21  & dust \\
SPICY 87918 & 279.1619 & -1.2247 &      31.5184 &      5.32671 & 484  & 11  &
 21  & dust \\
IRAS 18358-0112 & 279.6079 & -1.1642 &      31.6211 &      5.34537 & 482  & 12 
 & 16  & dust \\
2MASS J18391236-0720158 & 279.8015 & -7.3377 &      29.0540 &      4.01985 &
 252  & 10  & 10  & dust \\
IRAS 18383+0059 & 280.2154 & 1.0358 &      31.6859 &      5.34800 & 489  & 13  &
 13  & dust \\
IRAS 18440+0023 & 281.6343 & 0.4524 &      29.3592 &      3.97885 & 623  & 43  &
 33  & dust \\
IRAS 18454+0250 & 282.0028 & 2.9048 &      31.4409 &      4.48695 & 610  & 66  &
 72  & dust \\
SPICY 92856 & 282.4536 & 0.1079 &      25.2520 &     0.228420 & 628  & 22  & 22 
 & dust \\
2MASS J18494869+0006072 & 282.4529 & 0.102 &      29.1810 &      2.21213 & 628 
 & 22  & 22  & dust \\
SPICY 92905 & 282.4845 & 0.1893 &      25.2591 &     0.181341 & 627  & 24  & 26 
 & dust \\
SPICY 92890 & 282.4712 & 0.2159 &      29.1896 &      2.20579 & 627  & 24  & 26 
 & dust \\
IRAS 18484+0237 & 282.7392 & 2.6811 &      25.2462 &     0.161605 & 583  & 86  &
 43  & dust \\
GGD30IR & 282.9188 & 0.4828 &      25.2644 &     0.162153 & 611  & 42  & 20  &
 dust \\
MSX6C G034.0126-00.2832 & 283.6346 & 0.8594 &      30.1483 &      2.65985 & 606 
 & 16  & 20  & dust \\
MSX6C G034.0500-00.2977 & 283.6346 & 0.8594 &      30.3408 &      2.44161 & 606 
 & 16  & 20  & dust \\
HIGALBM G036.9422+01.1219 & 283.6902 & 4.0805 &      30.4409 &      2.48089 &
 547  & 18  & 13  & dust \\
IRAS 18528+0400 & 283.8458 & 4.0764 &      30.4549 &      2.44962 & 570  & 35  &
 35  & Gaia \\
HIGALBM G034.3721-00.5424 & 283.9992 & 1.0342 &      30.3426 &      2.35307 &
 603  & 20  & 23  & dust \\
AGAL G034.196-00.592 & 283.9632 & 0.8555 &      30.3599 &      2.25142 & 606  &
 16  & 22  & dust \\
HIGALBM G034.3395-00.6940 & 284.1192 & 0.9361 &      25.0171 &    -0.622316 &
 606  & 16  & 25  & dust \\
IRAS 18555+0056 & 284.5353 & 1.0116 &      32.6447 &      2.82884 & 605  & 21  &
 23  & dust \\
IRAS 18550+0104 & 284.4038 & 1.1356 &      32.6073 &      2.53868 & 606  & 19  &
 27  & dust \\
IRAS 18542+0114 & 284.2011 & 1.3131 &      33.0093 &      2.68810 & 588  & 31  &
 15  & dust \\
{[BCM2016]}~8a/G35.2-0.74N & 284.5543 & 1.6767 &      33.0082 &      2.29025 &
 2190  & 200  & 240  & maser \\
IRAS 18558+0047 & 284.5999 & 0.8649 &      32.7907 &      1.33449 & 605  & 21  &
 20  & dust \\
IRAS 18566+0048 & 284.8058 & 0.8775 &      33.0711 &      1.44530 & 606  & 24  &
 20  & dust \\
HIGALBM G038.6940+00.4527 & 285.0898 & 5.3335 &      33.0713 &      1.42530 &
 686  & 52  & 30  & dust \\
MSX6C G038.8750+00.3088 & 285.3017 & 5.4286 &      32.7720 &      1.26971 & 688 
 & 50  & 25  & dust \\
IRAS 18591+0503 & 285.3962 & 5.1303 &      34.4395 &      1.96140 & 690  & 40  &
 27  & dust \\
IRAS 18589+0511 & 285.3606 & 5.2574 &      35.0134 &      2.18817 & 690  & 44  &
 28  & dust \\
CORNISH G039.1956+00.2255 & 285.5232 & 5.6755 &      32.8665 &     0.473079 &
 686  & 56  & 24  & dust \\
HBC 684 & 286.7911 & 5.2197 &      35.2768 &      1.33091 & 696  & 35  & 23  &
 dust \\
IRAS 19045+0518 & 286.7488 & 5.382 &      33.2604 &     0.236187 & 699  & 54  &
 27  & dust \\
IRAS 19160+1139 & 289.6078 & 11.7472 &      34.1033 &    -0.325777 & 404  & 9  &
 11  & dust \\
IRAS 19158+1136 & 289.5513 & 11.6981 &      36.9101 &      1.10979 & 404  & 8  &
 10  & dust \\
AS 353 & 290.1291 & 11.0318 &      36.9318 &      1.11808 & 395  & 3  & 3  &
 Gaia \\
IRAS 19190+1048 & 290.3443 & 10.8992 &      36.9700 &      1.13113 & 405  & 5  &
 7  & dust \\
IRAS 18331-0035 & 278.9253 & -0.5557 &      36.9200 &     0.980824 & 484  & 15 
 & 20  & dust \\
Ser-emb 8 & 277.4504 & 1.2792 &      36.9836 &     0.986347 & 443  & 57  & 13  &
 dust \\
IRAS 18273+0113 & 277.4568 & 1.2561 &      34.4921 &    -0.396121 & 443  & 59  &
 13  & dust \\
Ser-emb 17 & 277.2758 & 0.512 &      34.0865 &    -0.634017 & 444  & 55  & 11  &
 dust \\
2MASS J18300341+0116191 & 277.5142 & 1.2719 &      34.4532 &    -0.454897 & 443 
 & 11  & 11  & Gaia \\
HH1183–1186 IRS1 & 290.1075 & 11.3331 &      34.2141 &    -0.720302 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS2 & 290.1077 & 11.3316 &      34.2384 &    -0.710613 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS3 & 290.1082 & 11.3356 &      34.2475 &    -0.713006 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS4 & 290.1085 & 11.3312 &      34.3296 &    -0.709312 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS5 & 290.109 & 11.3303 &      34.6404 &    -0.791946 & 405  & 6 
 & 7  & dust \\
HH1183–1186 IRS6 & 290.1113 & 11.3321 &      35.2179 &    -0.742390 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS7 & 290.1127 & 11.3365 &      34.4494 &     -1.15167 & 405  &
 6  & 7  & dust \\
HH1183–1186 IRS8 & 290.1138 & 11.3323 &      34.4874 &     -1.15886 & 405  &
 6  & 7  & dust \\
SSTc2d J192134.8+112123 & 290.3951 & 11.3565 &      34.6036 &     -1.12361 &
 405  & 6  & 7  & dust \\
\enddata
\tablenotetext{a}{Distances determined either from Gaia, dust maps \citet{Edenhofer24}, or maser-based parallax 
%in the case of G35.2-0.74N 
\citep{Zhang09}.} 
\end{deluxetable*}
